On LLMs-Driven Synthetic Data Generation, Curation, and Evaluation: A Survey

Within the evolving landscape of deep learning, the dilemma of data quantity and quality has been a long-standing problem. The recent advent of Large Language Models (LLMs) offers a data-centric solution to alleviate the limitations of real-world data with synthetic data generation. However, current investigations into this field lack a unified framework and mostly stay on the surface. Therefore, this paper provides an organization of relevant studies based on a generic workflow of synthetic data generation. By doing so, we highlight the gaps within existing research and outline prospective avenues for future study. This work aims to shepherd the academic and industrial communities towards deeper, more methodical inquiries into the capabilities and applications of LLMs-driven synthetic data generation.

==> sec/preliminary.tex <==
\section{Preliminaries}
\subsection{Problem Definition}
The automated data generation pipeline is driven by a pre-trained LLM $\mathcal{M}_{\theta}$ with parameter $\theta$. We are initially given a particular target task $\mathcal{T}$ with label space $\mathcal{Y}$ and an optional small reference set $\mathcal{D}_\mathit{ref}=\{(x_i,y_i)\}_{i=1}^{N}$ that can be either labeled or unlabeled.  The primary goal is to harness the capabilities of $\mathcal{M}$ to induce samples $(x^\mathit{gen},y^\mathit{gen})$ where $y^\mathit{gen}\in\mathcal{Y}$ and then constitute a synthetic dataset $\mathcal{D}_\mathit{gen}=\{(x_i^\mathit{gen},y_i^\mathit{gen})\}_{i=1}^{N_\mathit{gen}}$ :
\begin{equation}
    \mathcal{D}_\mathit{gen} \leftarrow G(\mathcal{M}_\theta, \mathcal{T}, \mathcal{D}_\mathit{ref})
    \label{eq:overall}
\end{equation}
where $G$ is the overall generation algorithm. Under this unified framework, the generation pipelines can be divided into two types: \textbf{data synthesis} and \textbf{data annotation}, which is illustrated in Figure~\ref{}.
\begin{itemize}
    \item \textbf{Data Synthesis} employs LLMs as generators to create new fictitious samples.  Given label-specific prompt, $\mathcal{M}$ is steered to generate multiple data $\{x_i^\mathit{gen}\}_{i=1}^{N_\mathit{gen}}$ for  targeted class $y^\mathit{gen}$. 
    \item \textbf{Data Annotation} employs LLMs as labelers to annotate the existing unlabeled data. Given an unlabeled set $\mathcal{D}_u$, $\mathcal{M}$ is prompted to predict the label $y^\mathit{gen}$ for each unlabeled sample $x_u\in \mathcal{D}_u$ and the input-label pair constitute $\mathcal{D}_\mathit{gen}$.
\end{itemize}
Notably, both of these two paradigms can be integrated with demonstrations from $\mathcal{D}_\mathit{ref}$ for boosted performance, which can be samples of target class for data synthesis and relevant input-label pairs for data annotation. This is known as \textbf{few-shot} setting, whereas \textbf{zero-shot} setting denotes the situation without demonstration samples from $\mathcal{D}_\mathit{ref}$. 


\paragraph{Requirements of $\mathcal{D}_\text{gen}$.} Distinguished from data generation in a broad sense, in this paper we only investigate methods that can provide supervision information valuable to other downstream tasks through data flow, which raises specific requirements to the generated $\mathcal{D}_\text{gen}$ from the following three aspects:

\begin{itemize}
    \item \textbf{Faithfulness.}
    To provide valid supervision, the generated data firstly should be not only correctly labeled, but also both logically and grammatically coherent.
    \item \textbf{Diversity.}
    Limited by the inherent bias of LLMs, the generated contents usually tend to be monotonous. However, the distribution of real data often exhibits a high degree of diversity, which should also be reflected in the generated data for better alignment.
    \item \textbf{Coverage.}
    Domain coverage is another essential element to ensure the robustness of deploying $\mathcal{D}_\text{gen}$ in the downstream tasks.
\end{itemize}

==> wfgpdzfdwdyxvfnvwdgfyvxthbhxjbsd/sec/0_abstract.tex <==
\begin{abstract}
Within the evolving landscape of deep learning, the dilemma of data quantity and quality has been a long-standing problem. The recent advent of Large Language Models (LLMs) offers a data-centric solution to alleviate the limitations of real-world data with synthetic data generation. However, current investigations into this field lack a unified framework and mostly stay on the surface. Therefore, this paper provides an organization of relevant studies based on a generic workflow of synthetic data generation. By doing so, we highlight the gaps within existing research and outline prospective avenues for future study. This work aims to shepherd the academic and industrial communities towards deeper, more methodical inquiries into the capabilities and applications of LLMs-driven synthetic data generation.
\end{abstract}

==> wfgpdzfdwdyxvfnvwdgfyvxthbhxjbsd/sec/1_introduction.tex <==
\section{Introduction}
The game-changing emergence of Large Language Models (LLMs) instigated a significant paradigm shift in the field of deep learning~\cite{abs-2303-11717,abs-2301-07597,abs-2302-04023}. 
Despite these advancements, a large amount of high-quality data remains the foundation for building robust NLP models~\cite{abs-2404-14361}. To be more specific, here high-quality data typically refers to diverse data that carries rich supervision signals (generally in the form of labels) closely aligned with human intent.
However, fulfilling such data reliance with human data can be challenging or even unrealistic sometimes, due to high costs, data scarcity, privacy concerns, etc. \cite{kurakin2023harnessing}. Moreover, several studies~\cite{abs-2309-16349,abs-2312-06585,abs-2303-15056} have highlighted that human-generated data, being inherently susceptible to biases and errors, may not even be optimal for model training or evaluation. These considerations necessitate a more serious inquiry into the question: are there other more \textit{effective and scalable} methods of data collection that can overcome the current limitations?

% {\color{red} Story here is kind of soft. While specialist SLMs are possible, general SLMs are also proven to be workable by the phi series. What is the secret sauce underlying the phenomenon that SLMs that achieve on par performance with models of much higher scale? -- High-quality training data (LLM-curated or LLM-synthesized data.}

Given the recent advancements in LLMs, which demonstrate the capability to generate fluent text on par with human output~\cite{hartvigsen-etal-2022-toxigen, sahu-etal-2022-data, ye-etal-2022-zerogen, abs-2303-04360, GaoPLXY0ZLLK23}, synthetic data produced by LLMs emerges as a viable alternative or supplement to human-generated data. Specifically, synthetic data is designed to mimic the characteristics and patterns of real-world data~\cite{abs-2404-07503}. On the one hand, LLMs, through extensive pretraining, have acquired a vast repository of knowledge and demonstrate exceptional linguistic comprehension~\cite{abs-2207-02516,ding-etal-2023-gpt}, which forms a foundation for generating faithful data. On the other hand, the profound instruction-following capabilities of LLMs allow better controllability and adaptability over the generation process, facilitating the creation of tailored datasets for specific applications with more flexible process designs~\cite{abs-2305-07759}. These two advantages make LLMs highly promising synthetic data generators.

\begin{figure}
\centering
\includegraphics[width=1\linewidth]{fig/Illustration.pdf}
\caption{Illustration of the LLMs-based application ecosystem, where synthetic data serves as the flowing nutrients for fruiting (training of small LMs or fine-tuning task-specific LLMs) and rooting (training stronger LLMs or self-improvement).}
\label{fig:illustration}
\end{figure}

% {\color{red} Another problem is that human-generated data is not necessarily optimal. To achieve superhuman agents, future models require superhuman feedback in order to provide an adequate training signal, where humane performance can instead be a bottleneck.}

% As a pivotal application of LLMs, synthetic data generation plays a crucial role in facilitating the dissemination of knowledge within the LLMs-based application ecosystem. 
As a pivotal application of LLMs, synthetic data generation holds significant importance for the development of deep learning. As shown in Figure~\ref{fig:illustration}, 
LLMs-driven synthetic data generation~\cite{LiZL023,wang-etal-2021-want-reduce,seedat2023curated} enables the automation of the entire model training and evaluation process with minimal human participation required in the loop~\cite{0001GHW00023}, which allows the advantages of deep learning models to be applied across a broader range of applications. Beyond providing a scalable supply of training and testing data, LLM-driven synthetic data generation also may pave the way for developing next-generation LLMs. Insights from TinyStories~\cite{abs-2305-07759} and the \textit{Phi} series~\cite{abs-2306-11644,abs-2309-05463} emphasize that data quality is crucial for effective model learning, while LLMs empower us to actively ``design'' what the models learn through data manipulation, significantly enhancing the efficacy and controllability of model training. 
% From another perspective, self-teaching with synthetic data generation is also a crucial step towards achieving superhuman intelligence~\cite{abs-2312-06585}, which requires superhuman feedback to provide an adequate training signal while human performance can instead be a bottleneck~\cite{abs-2401-10020}. 
As of June 2024, there are over $300$ datasets on Hugging Face\footnote{\url https://huggingface.co} that are tagged as ``synthetic'', with many mainstream LLMs leveraging high-quality synthetic data for training, including Alpaca~\cite{alpaca}, Vicuna~\cite{zheng2023judging}, OpenHermes 2.5, and Openchat 3.5~\cite{wang2023openchat}.

Though seemingly straightforward, 
% data synthesis with LLMs requires careful designs that encompass prompt engineering, process design, and data curation to obtain high-quality, diverse data, 
generating synthetic datasets that simultaneously have high correctness and sufficient diversity requires careful process designs and involves a lot of tricks~\cite{abs-2404-14361},
making LLMs-driven synthetic data generation a non-trivial problem. While most existing works generally target data generation for various tasks (e.g., pre-training~\cite{abs-2306-11644,abs-2309-05463,abs-2305-07759}, fine-tuning~\cite{abs-2306-02707,abs-2311-11045,abs-2304-12244}, evaluation~\cite{feng-etal-2023-factkb,abs-2403-18802}) across different domains (e.g., math~\cite{abs-2309-12284,abs-2308-09583}, code~\cite{abs-2306-08568,abs-2312-02120}, instruction~\cite{honovich-etal-2023-unnatural,wang-etal-2023-self-instruct}), they share many common ideas. To address the lack of a unified framework in the emerging field of LLM-driven synthetic data generation and develop a general workflow, this survey investigates recent studies and organizes them according to the topics of generation, curation, and evaluation, which are closely related, as shown in Figure~\ref{fig:taxonomy}. Our primary aim is to provide a comprehensive overview of the current state of the field, identify key areas of focus, and highlight the gaps that remain to be addressed. We hope to bring insights to both the academic and industrial communities and drive further development in LLM-driven synthetic data generation.

% Moreover, the absence of a unified framework in existing studies not only hinders in-depth systematic research but also poses significant barriers to its application in industrial settings. To this end, this paper mainly targets two classes of people: (i)-\textit{producers} who want to synthesize domain data faster and more efficiently, we summarize a systematic workflow for the industrial practice of LLMs-driven synthetic data generation, curation, and evaluation, as shown in Figure~\ref{fig:taxonomy}; (ii)-\textit{researchers} who are interested in data-centric AI \cite{mazumder2022dataperf}, we organize the recent literature to provide an overview of the current state of the field and highlight the gaps that remain to be solved.

% Notably, distinguished from common AIGC with generative models like GANs \cite{DBLP:journals/corr/GoodfellowPMXWOCB14,DBLP:conf/icmv/AissaMZ19} and Diffusion Models \cite{DBLP:conf/nips/HoJA20,DBLP:journals/csur/YangZSHXZZCY24}, here we only discuss synthetic data that can be applied to downstream tasks or are valuable for statistic analysis.

% in this paper, we formally propose a generic pipeline for LLMs-driven synthetic data generation and organize the recent literature to provide a systematic overview of the current state of the field. Meanwhile, through inductive analysis, we also highlight the gaps and limitations that remain to be solved, indicating the directions for further studies.

% In recent years, the rise of deep learning has driven advancements in various fields, leading the fourth industrial revolution \cite{goldblum2023perspectives,shoaib2023advanced,golroudbari2023recent}.
% part of its profound success can be attributed to the support of booming data, which plays an important role throughout the entire process of training, testing, and validation of neural networks. 
% Traditionally, such data are collected from the real world, followed by manual annotation to provide valid supervision aligned with human prior. Despite its simplicity, 
% With the expanding scale of deep learning models and their increasingly specialized applications, there is a demand for ever larger amounts of domain-specific data. Under such a situation, the availability of traditional human data is facing unprecedented challenges, being limited by the expensive human labor and demands for extra expertise involved during the data collection process \cite{}. 
% To be specific, 
% the limitation of human data begins to gradually emerge, which can be mainly manifested in insufficient \textbf{quantity} and unsatisfactory \textbf{quality}. 
% While adequate training data is often essential to reduce overﬁtting and enhance the robustness of deep learning models, the high cost of human labor and demands for extra expertise in specific tasks seriously limit the scalability of human-annotated data. Besides, collecting data from the real world may raise privacy concerns or even be legally constrained, further challenging human data collection. On the other hand, data collection is a noisy and rather unreliable process that involves numerous errors and biases in practice, where there are often signiﬁcant mismatches between the training and test distributions, leading to undesired learning effects. 

% To address this problem, there are two common strategies for mitigating the dependence on labeled data. One is to \textit{optimize data utilization} by methods including weakly supervised learning and unsupervised learning, etc. Despite their effectiveness, most of these methods are either highly task-specific or under strong assumptions, lacking enough universality. The other 
% Addressing this problem, 
% a natural idea is filling the gap in real data by \textit{artificially creating faithful ones}. As an early attempt, \textbf{data augmentation} synthesizes new examples from the existing ones with various heuristics or simple transformations,
% such as instance mixup, noise injection, and standard transformations
% while still requiring a certain amount of original data, and the quality of the synthetic data often cannot be guaranteed. As the development of generative models like GANs and Diffusion Models sheds light on the \textbf{unsupervised generation} of high-quality data, 
% some early studies in computer vision pioneer leveraging the generative models, such as GANs and Diffusion Models, to produce faithful images for downstream tasks. However, relevant research on text data has been seriously lagging behind due to the inherent semantic and grammatical complexity of natural language, 
% Recent works have noted that Large Language Models (LLMs) are capable of generating even more preferable data than those written or annotated by humans \cite{}, shedding light on addressing the scarcity of real data with generated ones \cite{}. Ideally, with their formidable prowess in understanding and generating human-like texts, LLMs are expected to provide an unlimited amount of customized data for different downstream tasks. However, with the difficulty of fully eliciting the inherent knowledge of LLMs, research at the current stage mainly focuses on how to better leverage the generative ability of LLMs and improve the quality of generated data, through appropriately designed synthesis, annotation, or curation (which are collectively termed as \textbf{synthetic data generation}). 
% As shown in the right half of Figure \ref{fig:illustration}, the generated data can be either deployed for training smaller domain-specific models or fed back to the LLMs for self-improvement. Figuratively speaking, the synthetic data serves as the flowing nutrients that transport knowledge between models, greatly facilitating the formation of an LLMs-based application ecosystem.

% Another significant impact of synthetic data generation with LLMs is that it revolutionizes the way that deep learning models interact with each other. 
% Compared with other model-centric methods for mitigating the dependence on labeled data (e.g., weakly supervised learning and unsupervised learning), the significance of synthetic data generation lies in its \textbf{greater universality and higher feasibility}. Specifically, the interactive nature of LLMs enables them to adapt to different scenarios, consequently allowing the generated data to cover a broader range of downstream tasks.
% % From a data-centric perspective, such a paradigm established specific knowledge pathways between the LLM and other models in the form of data flow. 
% As shown in Figure \ref{fig:illustration}, according to the available data resources, LLMs can be explicitly instructed to serve as data synthesizers, annotators, or curators, to generate data that can be deployed for either training of smaller domain-specific models or self-improvement of LLMs themselves, yielding a self-contained ``ecosystem'' wherein the synthetic data plays the role of flowing nutrients to transport knowledge between models.
% if we liken an LLM to an apple tree and synthetic data to the flowing nutrients within it, then upwards, it can bear high-quality fruits, namely \textbf{specialized smaller models} with more powerful functions tailored for various domains; downwards, it can be used for the \textbf{self-improvement} of the LLM, making the tree more deeply rooted and sturdy. With such a self-contained paradigm, we have reason to belive that the thriving of AI ecosystem is in the near future. 

% From a higher perspective, with data being a medium that xxx, the success of synthetic data generated by LLMs also symbolizes an important step towards 
% The idea of minimizing human participation in the process of data collection through extracting knowledge from the LLMs instead can also share insights with aligning the generative contents with human intentions.

% From a higher perspective, the significance of synthetic data generation not only lies in offering an economical alternative to minimize human participation in the development of AI systems, making it a (mostly) autonomous process with higher efficiency, but the success of generating data that can accurately reflect human intentions for supervisory purpose can also provide general insights on more controllable generation with LLMs.
% the success of synthetic data generation also signifies an important step towards the exploration in the industrial use of LLMs.


==> wfgpdzfdwdyxvfnvwdgfyvxthbhxjbsd/sec/2_preliminaries.tex <==
% \begin{figure*}
% \centering
% \includegraphics[width=1\textwidth]{fig/Taxonomy_Final.pdf}
% \caption{Taxonomy.}
% \label{fig:taxonomy}
% \end{figure*}

\section{Preliminaries}
\subsection{Problem Definition}
% In this paper, we investigate synthetic data generation specifically driven by a pre-trained LLM $\mathcal{M}_{\theta}$ with parameter $\theta$, where we are initially provided with an optional support dataset $\mathcal{D}_\text{sup}$ consisting of either labeled or unlabeled samples (cases where no labeled data is available are specified by the zero-shot setting). Our primary goal is to harness the capabilities of $\mathcal{M}_\theta$ to constitute a synthetic dataset $\mathcal{D}_\text{gen}$, which can be formulated as:
In this paper, we investigate the challenge of generating high-quality synthetic data using pre-trained LLMs, denoted as $\mathcal{M}$. Rather than creating new datasets from scratch, in more cases, we perform data augmentation with a small number of seed samples or unlabeled inputs, which we denote uniformly as $\mathcal{D}_\text{sup}$. Although optional for LLMs-driven synthetic data generation, $\mathcal{D}_\text{sup}$ can typically provide valuable supporting information when available. Consequently, the overall generation task can be formulated as:
\begin{equation}
    \mathcal{D}_\text{gen} \leftarrow \mathcal{M}_{p}(\mathcal{T}, \mathcal{D}_\text{sup})\text{,}
    \label{eq:overall}
\end{equation}
where $\mathcal{D}_\text{gen}$ represents the final generated dataset, and $p$ refers to the prompt used for model inference. $\mathcal{T}$ specifies the generation task, such as rewriting, question answering,  annotation, etc. Notably, data annotation as a specialized paradigm of synthetic data generation, has particularly extensive applicability, including RLAIF~\cite{abs-2212-08073} and LLMs-based evaluation~\cite{abs-2307-08701,zheng2023judging,abs-2310-08491}, which may involve specific challenges and corresponding solution techniques. Due to page limitations, further details about data annotation can be found in Appendix~\ref{app:data_annotation}.
% General data synthesis aims at creating fictitious samples with the help of LLMs. Among them, data annotation is an important and special case, where the $\mathcal{D}_\text{sup}$ specifically consists of a small number of labeled data that can be used as in-context demonstrations and mostly unlabeled data waited for annotation. Despite its particularity, data annotation shares the same basic ideas with common data synthesis. Therefore, in the following introduction, we will not deliberately distinguish between the two, while more particular details about data annotation can be referred to in Appendix~\ref{app:data_annotation}.

% Under this unified framework, the generation pipelines can be specifically divided into two types: \textbf{data synthesis} and \textbf{data annotation}, which is illustrated in Figure~\ref{fig:illustration}.
% \begin{itemize}
%     \item \textbf{Data Synthesis} employs LLMs as generators to create new fictitious samples. In this scenario, the generated data can either be in the traditional format with distinct input and label for tasks like classification and sentiment analysis, or it can be open-ended text pairs, and may even be samples without explicit differentiation between input and output (e.g., harmless instructions for model fine-tuning).
%     \item \textbf{Data Annotation} employs LLMs as labelers to annotate the existing unlabeled data. In this scenario, specifically, $\mathcal{D}_\text{sup} = \mathcal{D}_\text{l} \cup \mathcal{D}_\text{u}$ consists of mostly \underline{u}nlabeled data waited for annotation, while supported with a small number of \underline{l}abeled data that can be used as in-context demonstrations.
% \end{itemize}
% Notably, both of these two paradigms can be integrated with demonstrations from $\mathcal{D}_\mathit{ref}$ for boosted performance, which can be samples of target class for data synthesis and relevant input-label pairs for data annotation. This is known as \textbf{few-shot} setting, whereas \textbf{zero-shot} setting denotes the situation without demonstration samples from $\mathcal{D}_\mathit{ref}$. 

\begin{figure}[!t]
\centering
\includegraphics[width=1\linewidth]{fig/Taxonomy_2.pdf}
\caption{A taxonomy of LLMs-driven synthetic data generation, curation, and evaluation.}
\label{fig:taxonomy}
\end{figure}

\subsection{Requirements of $\mathcal{D}_\text{gen}$} 
\label{sec:requirements}
% The pursuit of downstream application value raises specific requirements for $\mathcal{D}_\text{gen}$, which can be summarized into the following three characteristics:
Briefly speaking, our goal is to generate data that closely aligns with evaluation metrics. While the standard of high-quality data may vary across different downstream tasks, there are two general requirements that are considered challenging in most existing literature:
\begin{itemize}
    \item \textbf{Faithfulness.}
    To provide valid supervision, the generated data must first be logically and grammatically coherent. However, the inherent problems of hallucination fat-tailed knowledge distribution of LLMs can introduce significant noise into the generated results, manifesting as factual errors, incorrect labels, or irrelevant content. These issues become more pronounced when generating long, complex, or domain-specific data.
    \item \textbf{Diversity.}
    Diversity captures the variation among the generated data, reflecting differences in text length, topic, or even writing style. It is crucial for generating synthetic samples that mimic the diversified nature of real-world data, thereby preventing overfitting and bias during model training or evaluation. Nevertheless, due to the inherent biases of LLMs, uncontrolled generated content often tends to be monotonous, limiting its applicability in downstream tasks.
    % \item \textbf{Coverage.}
    % Domain coverage is another essential element to ensure the robustness of deploying $\mathcal{D}_\text{gen}$ in the downstream tasks.
\end{itemize}
These two requirements are the focal points of most current research efforts. In the subsequent workflow, we will introduce how different methods address these issues.







% \subsection{Problem Definition}
% The initial goal of synthetic data generation is to obtain a high-quality dataset $\mathcal{D}_\text{gen}$ given an original set $\mathcal{D}_\text{ori}$ (if available). Powered by an LLM $\mathcal{M}$ with parameters $\theta$, we have:
% \begin{equation}
%     \mathcal{D}_\text{gen} = G(\mathcal{M}_\theta, \mathcal{T}, \mathcal{D}_\text{ori})
%     \label{eq:overall}
% \end{equation}
% where $\mathcal{T}$ and $G$ refer to the model inference task and the overall generation algorithm, respectively. 

% Distinguished from data generation in a broad sense, in this paper we only investigate methods that can provide supervision information valuable to other downstream tasks through data flow, which raises specific requirements to the generated $\mathcal{D}_\text{gen}$ from the following three aspects:
% \begin{itemize}
%     \item \textbf{Faithfulness.}
%     To provide valid supervision, the generated data firstly should be not only correctly labeled, but also both logically and grammatically coherent.
%     \item \textbf{Diversity.}
%     Limited by the inherent bias of LLMs, the generated contents usually tend to be monotonous. However, the distribution of real data often exhibits a high degree of diversity, which should also be reflected in the generated data for better alignment.
%     \item \textbf{Coverage.}
%     Domain coverage is another essential element to ensure the robustness of deploying $\mathcal{D}_\text{gen}$ in the downstream tasks.
% \end{itemize}
% \subsection{Common Settings}
% In most cases, the generated $\mathcal{D}_\text{gen}$ serves as an extension, enhancement, or refinement of a pre-existing dataset $\mathcal{D}_\text{ori}$, while in practice, such a starting set is not always available or accessible. Therefore, according to the availability of $\mathcal{D}_\text{ori}$, the generation tasks cater to two fundamental settings: \textbf{few-shot} generation and \textbf{zero-shot} generation. 
% % Despite that , the boundary between few-shot and zero-shot generation is getting blurred with the synthetic alternative, which will be further discussed in Section \ref{para:icl}.
% Notably, under the few-shot setting, the given $\mathcal{D}_\text{ori}$ can still be noisy, imbalanced, or even unlabeled, further diversifying the generation tasks concerning different resources. Among them, \textbf{autonomous annotation} is getting much attention for its extensive application value, where the LLM is leveraged as an annotator for labeling the given $\mathcal{D}_\text{ori}$, which consists of unlabeled data that are readily available. Being partially synthetic, the $\mathcal{D}_\text{gen}$ with generated labels also carries supervision information distilled from the LLM.
% % It should be noted that with the necessity of data generation, $\mathcal{D}_\text{ori}$ is generally of a small scale (so-called few-shot generation), however, the limitation of human data is never merely a matter of insufficient quantity. In real-world practice, data collection is rather a noisy process, leading to data with low quality such as imbalanced distribution, incorrect labels, or lack of specification. Without intense labor for task-specific processing, such raw data can hardly satisfy the ever-increasing data demands of deep learning development. 
% % Meanwhile, $\mathcal{D}_\text{ori}$ 
% % Specifically, providing that $\mathcal{D}_\text{ori}$ consists of mostly unlabeled data, $\mathcal{D}_\text{gen}$ can be the result of \textbf{autonomous annotation}, by simply leveraging the LLM $\mathcal{M}_\theta$ as an annotator. Generally speaking, the generated $\mathcal{D}_\text{gen}$ can serve as an extension, enhancement, or refinement of $\mathcal{D}_\text{ori}$.


% % Back to the task of generating high-quality data, another question is how should such ``high quality'' be exactly defined under the topic of synthetic data generation? Considering $\mathcal{D}_\text{gen}$ as an ideal alternative to real human data, a straight answer would be enough \textbf{human-likeness}, which can be specifically assessed from the following three aspects of \textbf{faithfulness}, \textbf{diversity}, and \textbf{coverage}. In terms of faithfulness, the generated data should be not only correctly labeled, but also both logically and grammatically coherent. Limited by the inherent bias of LLMs, the generated contents usually tend to be monotonous and thus need careful control for better diversity, while the requirements for coverage emphasize more on the completeness of the generated dataset.  All these properties together make the generated data better aligned with the real ones, ensuring its effectiveness in downstream tasks.
% % Correspondingly, existing research primarily focuses on optimizing different components provided in Eq. \ref{eq:overall} to improve the quality of the obtained $\mathcal{D}_\text{gen}$ from the above three aspects, such as prompt engineering that looks for more effective $\mathcal{T}$ and model tuning for enhancing the capability of $\mathcal{M}_\theta$ itself. 

% % \section{Overview}
% % \subsection{Perspective of Data Generation}
% % Speaking of the limitations of human data for the development of deep learning, it is crucial to recognize that it is not merely a matter of insufficient quantity. In addition, considering the diversity of data sources and their intended usages, which can be task-specific, structurally demanded, or with varying quality, etc., the need for synthetic data can be concretely underscored from the following three aspects.

% % \paragraph{Extension.}
% % Indeed, limited availability remains the most significant challenge currently faced by supervision data, while increasing training data size is often essential to reduce overﬁtting and enhance the robustness of machine learning models in various tasks. In many cases, the high cost of human labor and demands for extra expertise in specific tasks are two of the main factors that make the collection of human-annotated data not scalable. While unlabeled data are more readily available, their utility in model training is quite limited and challenging without explicit supervision direction. Besides, being human-related, collecting data from the real world may raise privacy concerns or even be legally constrained. \textcolor{blue}{The emergence of today's LLMs with remarkable cognitive abilities across a plethora of tasks makes artificially synthesizing high-quality labeled data for supervised learning possible, which may become an efficient as well as economical supplementary to alleviate the problem of data scarcity with unlimited generation number and relatively low cost.} Results from recent work also showed that LLMs are comparable with or even exceed human annotators on many annotation tasks, making it possible to replace large-scale manual annotation with a fraction of cost \cite{abs-2303-03953,HuangKA23a,abs-2303-15056}, which significantly enhances the efficiency of direct knowledge infusion from the wild into AI models by circumventing human intervention.

% % \paragraph{Enhancement.}
% % In the context of increasingly specialized deep learning applications attaching more particular requirements to data resources, datasets for general purposes may not be qualified to be directly employed for model training. For example, training on sensitive data may cause privacy leakage due to the risk of data memorization. Additionally, models with exceptional security requirements may also necessitate fine-tuning data intendedly designed to enhance model harmlessness.  In such scenarios, some research has employed LLMs to generate samples specifically aligned with particular usage for augmentation of existing datasets or dataset curation. Such capability of customizing datasets as desired significantly increases the flexibility of model training, unlocking the potential for more specialized or personalized applications of deep learning.

% % \paragraph{Refinement.}
% % In real-world practice, data collection is rather a noisy process, where there are often signiﬁcant mismatches between training and test distributions, leading to undesired training effects. Such noise is specifically evident in cases where some of the collected data may be incorrectly labeled, especially under demand for expertise in some domain-specific tasks. Imbalanced data distribution is also a common manifestation of low data quality, where instances of certain categories may be underrepresented in the collected dataset. More generally, this issue can be a chronic problem for tasks with constantly expanding output spaces, leading to severe underperformance on the underrepresented data slices due to the incorrect prior probability of predicting them. However, data generation with LLMs often offers greater controllability and stability thanks to their outstanding instruction understanding abilities, thereby ensuring the quality of the dataset. With specific validation techniques, the accuracy of synthetic supplementary for dataset refinement can be further improved, even surpassing human supervision in certain tasks.

% % \subsection{Perspective of AI Evolution}
% % While high-quality synthetic data can effectively serve as a straight alternative to human data, compared with other existing methods that also mitigate the dependence on labeled data, including semi-supervised learning, unsupervised learning, knowledge distillation, and data augmentation, etc., what makes LLM-powered data synthesis evolutional? Indeed, with the support of LLMs, there is a significant improvement in both the quality and efficiency of data generation. Coupled with their inherent simplicity, universality, and versatility, synthetic data are now able to achieve performance beyond the reach of other similar methods. Despite all these advantages, from a higher perspective, more essentially, LLM-synthesized data to some extent liberates the training of deep learning models from the constraints of external environments, ushering in a new era of AI self-learning in the following two ways.
% % \paragraph{Synergy between large and small models.}
% % Although LLMs have demonstrated their strong zero-shot performance in various linguistic tasks, it is difficult to fully exert the capacity of LLMs merely through prompting, making the effects of direct inference usually lag behind task-specifically fine-tuned small models \cite{abs-2302-10198,abs-2305-03514,QinZ0CYY23}. This implies that, in the current era where AI can provide advanced productivity, perhaps we need not only versatile LLMs but also models of lighter scale but with expertise in various fields, to maximize the effectiveness as well as efficiency of AI applications in certain domains. Just as mentioned above, one of the common usages of synthetic data is to produce domain-specific supervision for the training of smaller models, which can be viewed as a form of knowledge distillation or distribution shift towards target domains. It allows transparent synergy between large models and small models, which can be completely autonomous. In this way, model training no longer requires heavy human labor and becomes even scalable. We can say that synthetic data lowers the threshold for deploying deep learning models, effectively facilitating the coverage of AI technology in various domains.
% % \paragraph{Self-improvement of LLMs.}
% % Some research has also shown that LLMs can self-improve based on the synthetic data generated by themselves. For example, \cite{0001GHW00023} studies how an LLM is able to self-improve its reasoning ability using only input sequences from multiple NLP task datasets but no supervised data. With the powerful reasoning abilities of LLMs, we can also further explore the ``dark knowledge'' contained within real-world data, which can be fed back to the models themselves for fine-tuning towards better cognition. The success of such a self-learning paradigm possibly suggests that AI has acquired a capacity for self-evolution just like natural creatures. When AI is able to both horizontally expand and vertically deepen completely on itself, without any reliance on external intervention, we have reasons to believe that the emergence of an AI ecosystem is also in the near future.

==> wfgpdzfdwdyxvfnvwdgfyvxthbhxjbsd/sec/3_data_generation.tex <==
\definecolor{yellow_highlight}{RGB}{249,218,120}
\definecolor{blue_highlight}{RGB}{224,235,246}
\definecolor{red_highlight}{RGB}{245,191,196}

\begin{figure*}[!ht]
\centering
\includegraphics[width=1\textwidth]{fig/new_prompt_eg.pdf}
\caption{A toy example of effective synthetic data generation. The corresponding fields for \colorbox{yellow_highlight}{task specification}, \colorbox{blue_highlight}{conditions}, and \colorbox{red_highlight}{in-context demonstrations} are highlighted, while < > marks the switchable contents.}
\label{fig:prompt}
\end{figure*}

\section{Generic Workflow}
% \subsection{Preliminaries}
% Despite the seemingly readily available inputs of the generation algorithm as shown in Eq. \ref{eq:overall}, pre-generation tuning actually plays an important role in the overall optimization of the generation process, which can be developed from the following three aspects.
% \begin{itemize}
%     \item \textbf{Data Preprocessing.}
%     For $\mathcal{D}_\text{sup}$ not represented in natural language such as structured tabular data, sometimes we may need to convert them into a form that LLMs can understand so that they can be either effectively deployed for later model fine-tuning or embedded into the prompts. Except for simply molding tabular data into a sentence structure closely resembling natural language, 
%     \cite{zhao2023tabula} also explores techniques like token sequence compression and middle padding to further optimize the efficiency of data utility.
%     \item \textbf{Model Fine-Tuning.}
%     \item \textbf{Selective Annotation.}
% \end{itemize}

Existing studies on LLMs-driven synthetic data generation generally incorporate three main topics: generation, curation, and evaluation. Various approaches are employed within these aspects to collaboratively achieve optimal data generation.

\subsection{Data Generation}
% As the foundation of the entire system, the generation stage is responsible for eliciting the inherent knowledge of LLMs in the form of required data.
In this section, we systematically summarize some common practices for synthetic data generation with LLMs, which can be roughly divided into prompt engineering and multi-step generation. An overall illustration is provided in Figure~\ref{fig:prompt}.

% , which can be abstracted as:
% \begin{equation}
%     \mathcal{D}_\text{gen} = \mathcal{M}_\theta(P(\mathcal{T},\mathcal{D}_\text{sup}))
%     \label{eq:overall_generation}
% \end{equation}
% where $P$ refers to the prompt adopted for model reference with specified task $\mathcal{T}$ and given $\mathcal{D}_\text{sup}$.
\subsubsection{Prompt Engineering}
\label{subsubsec:prompt_engineering}
\label{subsec:prompt_engineering}
One of the greatest advantages of LLMs for synthetic data generation is their instruction-following capability, which contributes to great controllability \cite{Wang2023PandaLMAA,Radford2019LanguageMA}. Therefore, many approaches try to guide LLMs with heuristic prompts to enhance the faithfulness and diversity of the synthetic data~\cite{abs-2404-07503}. 

Empirically, an effective prompt generally contains three key elements: \textit{task specification} $e_\text{task}$, \textit{generation conditions} $e_\text{condition}$, and \textit{in-context demonstrations} $e_\text{demo}$, which are then collectively wrapped with a template $E$ into the form of natural instruction:
\begin{equation}
    % p \leftarrow P(\mathcal{T},\mathcal{D}) \\
    p(\mathcal{T},\mathcal{D}) \leftarrow E(e_\text{task},e_\text{condition},e_\text{demo})\text{.}
    \label{eq:instruction}
\end{equation}
As shown above, both the generation task $\mathcal{T}$ and the support dataset $\mathcal{D}$ will affect the design of $p$. Next, we will proceed to detail how each part of the prompt should be appropriately designed to accommodate various scenarios.

\paragraph{Task Specification.}
In traditional crowdsourced annotation scenarios, the recruited workers are commonly offered a codebook that specifies the necessary contexts, such as task purpose, data explanation, and other background knowledge, so that they can better understand their jobs \cite{abs-2303-15056}. Similarly, such task specification is crucial for setting the right context for LLMs-driven data generation, which can also include role-play~\cite{LiZL023}, format clarification, knowledge augmentation~\cite{abs-2311-00287,abs-2403-01081}, etc. Evidence shows that a simple prologue such as ``suppose you are a \texttt{\{xxx\}}'' can significantly improve the LLMs' performance by setting up a proper scenario for data generation and allowing the LLMs to better take on the roles \cite{LiZL023}. More formally, \citet{YooPKLP21} defines the task specification with a triplet of text type, label type, and label-token verbalizer. Such a description header is particularly important when extra domain expertise is demanded to address issues like terminology complexities in both context understanding and data generation. Consequently, \citet{abs-2311-00287} leverages external knowledge graphs and LLMs to obtain domain topics for context-informed prompting, which effectively enhances the faithfulness and complexity of generated data. 

% [TODO] Except for telling the LLMs \textbf{what} to do, such task specifications can also serve as guidance to the LLMs on \textbf{how} to generate better data. Among them, one of the most commonly used strategies is Chain-of-Thought (CoT) prompting, where we explicitly ask the LLMs to ``think step by step''. With such a series of intermediate reasoning steps, the ability of LLMs to generate complex data can be significantly improved \cite{Wei0SBIXCLZ22}. Besides, \citet{SahuVBL23} prompts the LLM with a deep mixup strategy, to generate more challenging samples.

\paragraph{Conditional Prompting.}
\label{para:conditional_prompting}
As mentioned in Section~\ref{sec:requirements}, a pivotal challenge in using LLMs for synthetic data generation is ensuring sufficient diversity, as directly prompting the LLMs to produce data for certain tasks often results in highly repetitive outputs, even with a high decoding temperature~\cite{abs-2404-14361,abs-2404-07503}. Addressing this problem, a widely adopted strategy is conditional prompting, which explicitly and concretely communicates to the LLMs the specific type of data desired.
The core of conditional prompting involves delineating the targeted data through the formulation of a series of condition-value pairs:
\begin{equation}
    e_\text{condition}=\{(c_1,v_1),(c_2,v_2),\cdots,(c_n,v_n)\}\text{,}
\end{equation}
which effectively characterizes the desired attributes and characteristics of the synthetic data.
With different combinations of such attributes, we can automatically achieve a degree of ``artificially defined'' diversity in the generated samples~\cite{abs-2306-11644,abs-2309-05463,abs-2305-07759}.
Conditional prompting not only allows better control over the diversity and coverage of the generated dataset but also refines the content to a narrower, more focused scope that is more likely to align with our specific expectations and requirements~\cite {LiZL023}. Current research on conditional prompting primarily centers on the following two subjects:
\begin{itemize}
    \item[1)] \textbf{Conditioning Scope.} As the backbone of $e_\text{condition}$, conditioning scope defined by $\{c_1,\cdots,c_n\}$ delineates the dimensions that we utilize to characterize our target data. Early studies \cite{GaoPLXY0ZLLK23,ye-etal-2022-zerogen,ye-etal-2022-progen} employed a basic output-conditional prompting strategy, utilizing the specific label associated with the classification task as the conditioning variable. The rationale behind this was primarily to maintain class balance and coverage. However, such a strategy is unsuitable for data lacking explicit category labels. Subsequent work by~\citet{abs-2306-15895} argues that conditional-prompting with finer-grained attributes (e.g., topics, length, and style \cite{abs-2311-00287}), can lead to more diversified generation due to the vast number of possible attribute combinations, being also applicable to open-ended data. Additionally, \citet{abs-2305-07759} also condition each generation on the task of incorporating three randomly chosen words into the generated story. This approach was also proven to significantly enhance the diversity of the generated data, shifting the focus from the heuristic features of the output to a more structured and targeted conditioning mechanism by adding ``creative randomness'' to the prompt~\cite{abs-2305-07759}.
    \item[2)] \textbf{Conditioning Values.} After defining the conditioning scope, we then need to assign concrete values to each condition. 
    % To generate a complete and balanced $\mathcal{D}_\text{gen}$, diversity and coverage should be synchronously ensured in terms of the conditioning instances. 
    Despite the seemingly straightforward strategy of sampling from the known classes or labels \cite{ye-etal-2022-zerogen}, there are cases where such an instance pool is unavailable. Addressing this problem, \citet{JosifoskiSP023} actively retrieves the conditioning instances from external knowledge graphs, while \citet{abs-2311-00287,ding-etal-2023-enhancing} leverage the LLMs to generate diversified instances for conditional prompting. Specifically, \citet{ding-etal-2023-enhancing} construct a concept tree to delve into different subtopics, ensuring the coverage of sampled conditioning values, which then contributes to more diverse generated data. Moreover, the prompt template $E$ can also be considered a special type of condition. It has been demonstrated that incorporating templates with a certain level of randomness throughout the generation process can enhance the diversity of the generated contents \cite{DBLP:conf/nips/MengHZH22}. 
\end{itemize}

\paragraph{In-Context Learning.}
\label{para:icl}
Due to the inherent bias of LLMs, it remains challenging to elicit favorable responses from the LLMs with merely task specification and conditional prompting. In this case, a straightforward yet effective strategy is to provide several demonstrations, which can serve as a form of implicit human guidance. Research has shown that, owing to LLMs' remarkable in-context learning (ICL) capabilities, a few exemplars can provide them with insights into the patterns exhibited in real-world data, thereby significantly improving the faithfulness of generated data \cite{LiZL023}. In the few-shot setting, where labeled samples are available in the support set $\mathcal{D}_\text{sup}$, these samples can be directly utilized as demonstrations for ICL. However, in scenarios where no ground truth data is available, approaches like Self-Instruct \cite{WangKMLSKH23} and Self-Prompting \cite{abs-2212-08635} instead leverage ICL with synthetic demonstrations generated by LLMs. This allows the models to learn from their own predictions or other teacher models, even in the absence of labeled data.

However, given the constraint of prompt length and data inconsistency, the quality of in-context samples significantly affects the effectiveness of in-context learning. \citet{abs-2403-01081} argue that randomly selecting in-context examples from the pool of seed samples, as done in Self-Instruct~\cite{WangKMLSKH23}, results in a lack of diversity and quality in the generated data. To address this issue, \citet{abs-2403-01081} opt for selecting examples that concentrate on specific aspects to better stimulate the long tail of knowledge inherent in LLMs. \citet{LiuSZDCC22} and \citet{SuKWSWX0OZS023} prioritize consistent samples as demonstrative examples based on their cosine similarity in the embedding space. Alternatively, \citet{ye-etal-2022-progen} selects the most informative samples using quantified influence scores to steer the generation process. To enhance the informativeness of in-context examples, \citet{abs-2303-16854} prompts LLMs to provide an explanation for each sample before integrating it into the prompt. This approach not only offers valuable additional information but also aligns well with the subsequent Chain-of-Thought generation.

% \paragraph{Prompt Template.}
% As the backbone of the instruction as shown in Eq. \ref{eq:instruction}, \textbf{prompt template} $T$ can also affect the generation performance to some extent, while \cite{} puts forward a general idea that using templates with a certain degree of randomness for prompting throughout the generation process can improve the diversity of the generated contents. 

\subsubsection{Multi-Step Generation}
% {\color{red} Is it better to use ``process design'' instead?}
In the previous paragraphs, we have introduced some common prompting strategies, which are typically designed for a specific generation task $\mathcal{T}$. However, in most cases, due to the lack of enough reasoning abilities, it is unrealistic to expect the LLMs to generate the entire desired dataset within a single reference, especially when targeting data with complex structures or semantics~\cite{abs-2310-04484}. 
% Generally speaking, this is because LLMs are naturally biased and lack enough reasoning capabilities, for which a measure of human intervention is necessary to obtain datasets that are well aligned with our favor, while guidance provided by a single prompt is insufficient. 
In addressing this problem, a common strategy is multi-step generation, through which the overall generation process is manually decomposed into a chain of simpler sub-tasks $\mathcal{T}_{1:k}$, to force the LLMs to produce data in a step-by-step manner as scheduled:
% where the overall generation pipeline is explicitly decomposed into multiple simpler stages, denoted by a task set $\bm{\mathcal{T}}=\{\mathcal{T}_0,\mathcal{T}_1,\cdots,\mathcal{T}_k\}$ that consists of $k$ sub-tasks. Correspondingly, the overall generation process in Eq. \ref{eq:overall} can be reformulated as follows:
% \begin{gather}
\begin{equation}
\begin{aligned}
    % &\mathcal{D}_\text{gen} &\leftarrow& \mathcal{M}_{\theta;p_k}(\mathcal{T}_k,\mathcal{D}_{k}) \\
    % &\mathcal{D}_{i+1} &\leftarrow& \mathcal{M}_{\theta;p_i}(\mathcal{T}_{i},\mathcal{D}_{i}), \ i=0,\cdots,k-1 \\
    % &\mathcal{D}_0 &\leftarrow& \mathcal{D}_\text{sup}
    % \mathcal{D}_{i+1} \leftarrow \mathcal{M}_{\theta;p_i}(\mathcal{T}_{i},\mathcal{D}_{0:i}), \ i=0,\cdots,k-1 \\
    % \mathcal{D}_0 = \mathcal{D}_\text{sup}
    \mathcal{D}_{i} \leftarrow \mathcal{M}^{i}_{p_i}(\mathcal{T}_{i},&\mathcal{D}_{0:i-1}), \ i=1,2,\cdots,k\text{,}
\end{aligned}
\label{eq:multi-step}
\end{equation}
% \end{gather}
% where intermediate outputs $D_{1:k}$ are sequentially produced to guide the generation in the next iteration until $\mathcal{D}_\text{gen}$ is obtained. Being more specifically defined, each sub-task is of less reasoning complexity, for which the LLMs are more likely to generate high-quality content. Notably, prompt design for each $p_i$ follows the same patterns as introduced in the previous section.
where $\mathcal{D}_0=\mathcal{D}_\text{sup}$. Each intermediate output $\mathcal{D}_i$ is generated using model $\mathcal{M}^i$, prompted by $p_{i}$, for a sub-task $\mathcal{T}_{i}$. These outputs can then potentially be used in subsequent generations. By manually scheduling the generation procedure, we implicitly align the reasoning paths of LLMs with human prior knowledge.
% Meanwhile, the previously overwhelming reliance on a single inference is now reasonably distributed with the introduction of sub-tasks, while prompts arising at different stages of generation also provide better accessibility for human control.
Specifically, there are two common strategies for task decomposition: \textit{sample-wise} and \textit{dataset-wise} decomposition, which mainly aim at enhancing the quality of synthetic data at different scales.
% In practice, such a fundamental paradigm of multi-step generation significantly enhances the effectiveness of the generated data and can also be considered as a form of human knowledge injection, where hints about the rationale behind data generation are dropped for the LLMs in the human-designed tasks $\mathcal{T}_{1:k}$ along with the generation pipeline.

\paragraph{Sample-Wise Decomposition.} A typical use-case of multi-step generation is for addressing the challenges of long-text processing and logical reasoning when dealing with multi-text data such as dialogues and entity-relation triplets. In such cases, a straightforward approach is to divide the sample into smaller chunks and generate only a portion of each sample at a time \cite{abs-2212-08635,ye-etal-2023-generating,WangKMLSKH23}. In this way, $\mathcal{D}_{1:k}$ can be considered as different parts of $\mathcal{D}_\text{gen}$:
\begin{equation}
    \mathcal{D}_\text{gen} = (\mathcal{D}_1,\mathcal{D}_2,\cdots,\mathcal{D}_k)\text{.}
\end{equation}
Notably, as shown in Eq.~\ref{eq:multi-step}, each iteration of the generation process can be conditioned on the previously generated contents. For example, \citet{ding-etal-2023-enhancing} prompts the LLMs to alternate between acting as the assistant and the user, replying to each other based on the context, ultimately producing a complete conversation transcript. In this way, the coherence among each internal component $\mathcal{D}_i$ can be pointedly reinforced with separated instructions, thus making it easier for the model to follow the requirements and generate more faithful data. It should be noted that $D_{1:k}$ may not necessarily form part of the final $D_\text{gen}$, instead, explicitly outputting some intermediate reasoning steps can also improve the generation of complex data \cite{abs-2212-08073,abs-2303-16854}. Chain-of-Thought (CoT) prompting stands out as one of the most popular strategies for improving the faithfulness of LLM-generated content~\cite{Wei0SBIXCLZ22}. Nevertheless, current research on the exploration of such latent metadata is still insufficient, leaving sample-wise task decomposition from a reasoning perspective an open problem for future studies.

\paragraph{Dataset-Wise Decomposition.}
% Considering that our goal is to generate a dataset that is closely aligned with the real-world distribution, a certain degree of human intervention over properties such as diversity and coverage of the overall data is often necessary. 
In Section~\ref{para:conditional_prompting} we have introduced how to generate data with specified properties. However, generating a series of such data that can eventually form a dataset with good diversity and domain coverage requires long-term scheduling. To this end, dataset-wise task decomposition dynamically adjusts the conditions used at each stage of multi-step generation to ensure the overall dataset grows in the right direction:
% appropriate long-term task decomposition.With appropriate adjustment of the conditions set in each stage of multi-step generation that complement each other as a whole, we can thus make the generated samples form a dataset with good diversity and coverage:
\begin{equation}
    \mathcal{D}_\text{gen} = \bigcup_{i=1}^{k}\mathcal{D}_i\text{.}
\end{equation}
Specifically, S3 \cite{WangZS23} targets the most frequently mislabeled categories at each iteration, according to the performance of the downstream model trained on previously generated data. 
Similarly, \citet{HonovichSLS23,ShaoGSHDC23} utilize a generate-then-expand paradigm, to enhance the diversity of the overall dataset accordingly. Some other methods also leverage specific data structures to model the pathways of data generation. For example, Explore-Instruct \cite{WanHYQB023} models the domain space as a tree structure and continually refines the generated data along with tree traversal to promote both the specialization and domain coverage of the generated data. 

% \paragraph{[Old] Heuristic Methods.}
% The key to multi-step generation is to appropriately define the generation task at each stage so that it can provide valuable guidance for the subsequent generation and eventually lead to a more reasonable $\mathcal{D}_\text{gen}$. For multi-text data generation, \citet{abs-2212-08635,DBLP:conf/emnlp/YeLK023,WangKMLSKH23} \textit{sequentially generate different parts of a sample}, each of which is also used as the prior to generate the remaining parts. Such multi-step generation can significantly help to improve the inherent consistency of the generated sample by heuristically setting a generation sequence that aligns with human knowledge while also shortening the span of reasoning. 
% S3 \cite{WangZS23} instead repeats the same generation task but with \textit{different prompting conditions} targeting the most frequently mislabeled categories according to the performance of the downstream model trained on previously generated data. 
% Similarly, \citet{HonovichSLS23} and \citet{ShaoGSHDC23} add a second round of generation to expand or reinforce upon the results of the previous generation.

% \paragraph{Systematic Modeling.}
% Recent studies have also 
% \textit{leveraged specific data structures to model the pathways of data generation}. For example, Explore-Instruct \cite{WanHYQB023} models the domain space as a tree structure and continually refines the generated data along with tree traversal to promote both the specialization and domain coverage of the generated data. 

% Another important trend in pipeline design is to \textit{combine data generation with other deep learning frameworks}, where external models in addition to $\mathcal{M}_\theta$ are introduced to process the intermediate generated products and derive the final $\mathcal{D}_\text{gen}$. \citet{abs-2205-02318} leverages heuristic prompts to extract various properties of the given sample rather than direct annotation, which are then provided for a standard weak-supervision framework to distill the ground truth label. 



% \cite{WangKMLSKH23} finds that ICL with the model-generated examples in previous steps can also promote the diversity of the generated data.

% Synthetic Prompting \cite{ShaoGSHDC23} alternates between a backward and forward process to generate high-quality data, which ensures that the question is both answerable and well-deﬁned and reﬁnes the reasoning chain to be more precise and consistent with the question, respectively.

% \section{Data Generation}
% % \subsection{Problem Definition}
% % \paragraph{Goals.}
% % high quality, human-like, close to real distribution, how to define? 
% % In order to make the generated synthetic data a better replacement for real data, it should be
% % \begin{itemize}
% %     \item \textbf{Faithfulness.}
% %     \item \textbf{Diversity.}
% %     \item \textbf{Coverage.} Retrieval Methods (from databases, knowledge graphs or other datasets), Tree Traversal (Knowledge Construction)
% % \end{itemize}

% % \paragraph{Settings.}
% \subsection{Prompt Engineering}
% One of the greatest advantages of LLMs for synthetic data generation is their outstanding controllability, mainly attributed to their powerfulness of instruction-following. Therefore, a large amount of research has focused on how to effectively prompt the LLMs to generate data well aligned with our demands. ZeroGen \cite{YeGLXF00K22} pioneers the generation-based zero-shot learning paradigm, where a pseudo synthetic dataset is generated with the simple label-descriptive prompt to train a \textbf{T}iny t\textbf{A}sk \textbf{M}odel (\textbf{TAM}) to solve the target task. However, there usually remains a gap between the distributions of synthetic data and real-world data. Fitting on such low-quality data will greatly hamper the performance of the task-speciﬁc model, making it unreliable for deployment \cite{}. Addressing this problem, the goals of prompt engineering can be further specified as improving the human-likeness of the generated data in terms of \textit{faithfulness}, \textit{diversity} and \textit{coverage}.

% \subsubsection{Prompt Elements} 
% To provide effective and comprehensive instruction, a complete prompt generally integrates the following four elements: \textit{contexts}, \textit{conditions}, \textit{demonstrations}, and \textit{control information}, each of which guides data generation in different ways.

% \paragraph{Contexts.}
% In practice, human annotators are usually provided with codebooks about detailed task descriptions including information on task deﬁnition, task purpose, category standard, etc., so that the crowd workers are able to quickly acquire the basic demands of the task and thus better complete their jobs \cite{abs-2303-16854}.
% In the same vein, providing necessary background knowledge about the generation objective can encourage the LLMs to generate synthetic data that resemble the real texts produced in the targeted domain \cite{LiZL023}, or improve their annotation accuracy. 

% \cite{YooPKLP21} uses the triple of the meta information: text type $T$, label type $L$ and label-token verbalizer $v:\mathcal{Y}\rightarrow\mathcal{V}$, to form the task specification $S_\mathcal{T}=(T,L,v)$ for every task $\mathcal{T}$, allowing the large-scale language models to generalize better about the targeted distribution. \cite{abs-2309-00267} experiments on the ``OpenAI'' type of context prompting, which closely mimics the rating instructions given to the human preference annotators that generated the OpenAI TL, and achieves better performance on most of the setups compared to the ``Base'' type of context prompting. Such a description header is especially crucial in some domain-specific tasks that demand extra expertise to address issues like terminology complexities \cite{abs-2311-00287} and tasks wherein fine-level descriptions aligned with natural language are needed for unnatural labels (e.g., category labels in the RE task) \cite{ZhangLMZ023}. Correspondingly, \cite{abs-2311-00287} leverages both external knowledge graphs as well as LLMs to generate domain topics for context-informed prompting, integrating both non-parametric insights from external KGs and the intrinsic parametric knowledge encoded in LLMs. to generate high-quality data for training multilingual dense retrieval models, \cite{abs-2311-05800} proposes SAP (summarize-then-ask prompting), leveraging the LLM to generate a textual summary prior to the query generation step which is then used as the context to prompt the subsequent generation and can significantly improve the faithfulness of the generated data. \cite{abs-2305-03047} also offer a small set of 16 human-written principles about the desirable quality of the system-produced responses, or the rules behind the behavior of the AI model in producing answers in the prompt, which serve as guidelines for the LLMs to generate helpful, ethical, and reliable responses. 

% \paragraph{Conditions.}
% To better control the diversity and coverage of the synthetic data, manually specified conditions are generally integrated into the prompt to explicitly instruct data generation with specific style, label (concerning the classification task of interest), or other properties \cite{LiZL023}. 

% Being able to directly affect the distribution of the generation results, such conditions should be carefully designed for the synthetic data to be valuable. \cite{JosifoskiSP023} obtains the output triplet sets used for conditioning from external KGs, following specially designed sampling rules that encourage both coherence and coverage of the selection procedure. \cite{abs-2311-00287} also leverages writing styles drawn from LLMs to guide data generation, exploiting the creativity of LLMs to increase the diversity of conditional variables. Such conditions can also be selected based on the refinements of the previously generated data. For instance, \cite{WangZS23} uses the LLMs to extrapolate the errors of the small model and synthesize additional data of categories that are most frequently misclassified. To further diversify the generated data, \cite{abs-2306-15895} argues that simple class-conditional prompts applied in \cite{} may limit the diversity of the generated data and inherit systematic biases of LLMs. Thus, they investigate prompts with finer-grained attributes (e.g., topics, length, and style as applied in \cite{abs-2311-00287}), which provide a more specific description of the desired data and have the potential to yield more diversely attributed generated data. Experimental results show that adding more meta-information into the data generation prompts can effectively remove the bias in the generated synthetic data and improve the diversity of those synthetic data.

% It is noteworthy that appropriately specifying the inputs or outputs as conditions can also allow us to circumvent the challenges of structured generation by exploiting external knowledge bases in the manner of conditional prompting \cite{JosifoskiSP023} and improve the performance of auto-regressive regeneration by following the customary order of natural language expression, making the choice between data synthesis and annotation (which can be seen as data synthesis conditioned on the input texts) more flexible. 
% % Additionally, when considering whether to use the inputs or the outputs as the conditions, a well-designed conditional prompt should also adhere to natural language expression conventions from the perspective of auto-regressive generation \cite{abs-2109-09193,WangKMLSKH23}. [TODO: Move to pipeline design]
 
% \paragraph{Demonstrations.}
% Due to the remarkable \textbf{I}n-\textbf{C}ontext \textbf{L}eaning (\textbf{ICL}) of LLMs, giving a very small amount of exemplars can provide LLM with insights of the patterns exhibited in the real-world data and thus significantly improve the faithfulness of the generated data \cite{LiZL023}. 

% Under the few-shot setting where a golden support set consisting of a few labeled samples is available, we can directly use them as demonstrations to boost the performance of data generation. Under the zero-shot setting where no labeled data are available, approaches like Self-Instruct \cite{WangKMLSKH23} and Self-Prompting \cite{abs-2212-08635} instead leverage ICL with demonstrations generated by the LLMs themselves. 

% However, constrained by the limited prompt length and data inconcsistency, given a demonstration pool, we can only select a part of it as in-context examples. Therefore, a set of works studies the strategies of how to the most informative demonstrations to unleash the LLMs' few-shot capabilities and further improve their performance. \cite{ZhangLMZ023} adopts the $k$-NN algorithm to select samples from a demonstration pool while \cite{YeG0F0K22} sorts the samples based on their quantiﬁed inﬂuence score and then formulates those most inﬂuential ones as in-context examples to steer the generation. For annotation tasks, inspired by the observation that in-context examples that are closer to the test sample in the embedding space consistently give rise to stronger performance (relative to the farther ones), \cite{LiuSZDCC22,SuKWSWX0OZS023} compute embeddings for all annotated samples using Sentence-BERT and use the most similar examples to each unlabeled instance in terms of cosine similarity as its corresponding in-context examples. However, \cite{ShaoGSHDC23} argues that according to \cite{FuPSCK23}, selecting demonstrations based on complexity can improve the performance of the model on reasoning tasks, compared to selecting them based on similarity. 
% % Moreover, selecting demonstrations based on similarity may introduce biases (Zhang et al., 2022b; Lyu et al., 2022) from the demonstrations, especially if they are incorrect. Furthermore, selecting demonstrations that are complementary to each other may help the model fuse knowledge from different types of reasoning (Ye et al., 2022b; Zhang et al., 2022b).
% Therefore, \cite{FuPSCK23} instead proposes an in-cluster complexity-based scheme to select demonstrations that are both complex and complementary. Except for improving the faithfulness of generated results, 

% % The order in which candidates are shown to the LLM can bias which candidate it prefers \cite{abs-2309-00267}
% % preprocessing \cite{BorisovSLPK23}
% % tabular data preprocessing: Token Sequence Compression, Middle Padding \cite{abs-2310-12746} [TODO: Move to pipeline design as data preprocessing] 

% \paragraph{Control Information.}
% In addition to all the prompt contents above that describe ``what kind of jobs does the LLM need to do'', we also need some control information to tell the LLM ``how is it supposed to get the jobs done'', through which we can transmit certain human behavior patterns or heuristic knowledge to the LLM to help them perform better. 

% One of the most commonly used strategies is Chain-of-Thought (CoT) prompting, where we explicitly ask the LLMs to ``think step by step'', simulating the way humans explain problems. With such a series of intermediate reasoning steps the ability of large language models to perform complex reasoning can be significantly improved \cite{Wei0SBIXCLZ22}. We can also apply this technique to the construction of in-context demonstrations. Specifically, \cite{abs-2303-16854} proposes an ``Explain-then-Annotate'' pipeline, where the LLMs are first leveraged to automatically generate reasonable explanations for demonstrated examples, which together with the human written rationales are used as in-context samples to elicit the LLMs' reasoning ability and thus increase the correctness of the generated data. \textcolor{blue}{natural language expression (with verbalizer) rather than label?}

% Besides, except for directly asking the LLMs to generate synthetic data, there are also many other tricks that can guide the LLMs to produce more valuable samples in an indirect way. For example, intuitively it would be easier for the LLMs to generate valid data by imitating the existing in-context examples than completely synthesizing from scratch. Therefore, \cite{abs-2307-16833,abs-2305-15041,abs-2304-12244} leverage different manually-designed prompts to explicitly instruct LLMs to rewrite the existing simple examples into more complex ones using in-depth methods (i.e., including more information on particular topics) or in-breadth methods (i.e, improving topics/information coverage). Moreover, to keep the LLM from producing homogeneous samples, an additional prompt is used in \cite{LiZL023} to impose a constraint on the LLMs in generating the synthetic data (i.e., ``You should imitate the example I have provided, but you cannot simply modify or rewrite the example I have given.''), while \cite{SahuVBL23} adopts a deep mixup strategy to generate more challenging samples near class boundaries by explicitly telling the LLMs to combine the features of different provided examples.

% % paraphrase, multi-target, story-telling \cite{abs-2307-16833}
% % Other methods instead ask the LLMs to generate contents that are more closely aligned with the natural language corpus, followed by further extraction methods to reform them into valid training samples. For example, \cite{abs-2307-16833} [TODO: Move to pipeline design?]

% % taxonomy-based generation \cite{abs-2305-15041} [TODO: Move to pipeline design]

% % synthesis or annotation?

% Soft Prompt: we start by tuning a set of parameter-efficient soft prompts for each of the attributes present in the seed data \cite{ChenLLRY23}

% \subsubsection{Prompt Construction}
% Another important part of prompt engineering is how to integrate all the above elements into a coherent whole. A well-designed prompt construction procedure can maximize the effectiveness of each component while enhancing the overall generalizability of the data generation method across various tasks.

% \paragraph{Prompt Templates.}
% Since prompts are typically presented in natural language, structural templates are required to connect all the disparate elements into clear and logically coherent passages. This is to ensure that the LLMs can clearly understand what each part of the prompt signifies, while also aligning the model's input as closely as possible with the distribution of natural language corpora in order to improve the performance of auto-regressive generation. Generally, a framework with placeholders that can be substituted with different task-specific elements will be provided as shown in Figure xxx, which can enable full automation from element selection to prompt construction. \cite{} also indicate that using different templates for prompting can significantly improve the diversity of the generated contents. It should be noted that such templates can also be dynamically updated throughout the process of data generation. \cite{LiZL023} provide a ``diversity prompt'' to the LLMs (i.e., ``Can you provide something more diverse compared to the previously generated data?'') after a few steps of generation, aiming to increase the diversity of the synthetic data. 

% % \paragraph{Condition Ensemble}
% % Instead of directly pretending xxx We then introduce a novel method for combining the Mixture of Soft Prompts (MSP) to generate diverse, class-conditioned training data in a carefully controlled manner. \cite{ChenLLRY23}

% % \paragraph{Dynamic Update.}


% \subsection{Model Tuning}
% Another way to improve the quality of data generated is by model fine-tuning. Though compared to prompt engineering in a relatively heuristic way, model tuning requires a much larger amount of computational resources while being also data-intensive, and is usually constrained by model accessibility, the fine-tuning approaches have their own advantage in improving the usability of the LLMs, such as enabling direct generation of high-quality data 
% % that are well-aligned with the helpful, ethical, and reliable principles across a wide range of queries 
% without the need to explicitly provide relevant principle set or ICL exemplars \cite{abs-2305-03047}. Additionally, being data-driven, model tuning is also able to make use of the knowledge embedded in data that is difficult to capture by heuristic methods. This series of methods typically involves work in the following three aspects.

% \paragraph{Model Selection.}
% Unlike prompt engineering, model tuning can be highly model-dependent, where both the difficulty and effect of fine-tuning can vary a lot on different models. Therefore, choosing an appropriate base model according to the task requirements is a very important first step in the tuning process. 

% Currently, there are two mainstream types of LLMs, one is the black-box Language-Model-as-a-Service (LMaaS) represented by the ChatGPT series, and the other is the open-source white-box models including HugginChat, LLaMA and FLAN. In the field of model fine-tuning, open-source LLMs are gaining more attention for their cost-effectiveness, transparency, reproducibility, and superior data protection that are typically not provided by commercial models \cite{alizadeh2023open}. With public access to the architectures and parameters of open-source LLMs, they can be easily scrutinized, tailored, and enhanced by a wider user base, for which we would have more options to directly apply the existing mature fine-tuning techniques for white-box models to make them better data generators. Though a relatively smaller parameter scale does limit their performance on some complex tasks to some extent, \cite{alizadeh2023open} shows that open-source LLMs not only outperform human-based services such as MTurk but also demonstrate competitive potential against ChatGPT in some specific text-annotation tasks. While black-box models like ChatGPT have demonstrated dominantly high performance across numerous NLP tasks, the opacity of parameters severely limits our ability to fine-tune them. Although some derivative-free optimization techniques have been recently proposed to optimize the continuous prompt prepended to the input text \cite{sun2022black}, direct fine-tuning of the black-box models remains unexplored territory. 
% % It should be noted that the different architectures of LLMs can also affect our choice of fine-tuning strategies as well as the effectiveness of the tuning. \cite{kumar2020data} compares the auto-regressive models and auto-encoder models on different benchmarks, and finds that 

% It should be noted that a properly initialized model can also greatly affect the effectiveness of fine-tuning. For specific instance, \cite{zhao2023tabula} advocates the use of a randomly initialized language model (instead of pre-trained ones) for tabular data synthesis, which can converge more rapidly compared to starting from a model extensively trained on irrelevant textual contents from books.

% \paragraph{Tuning Materials.}
% As we know, model tuning usually requires a large amount of labeled data which can be infeasible in some real-world scenarios. Similarly to the generation of demonstrations in prompt engineering, the scarcity of fine-tuning data can also be alleviated by data generation with LLMs. \cite{abs-2305-03047} fine-tunes the original LLM (the base model) on the self-aligned responses, generated by the LLM itself through prompting.

% \paragraph{Tuning Strategies.}
% After obtaining the base model and tuning materials, the next step is to choose appropriate strategies for targeted fine-tuning of the model. Beyond conventional fine-tuning methods, challenging NLU tasks can have largely similar distributions across different labels, with very nuanced differences reﬂected by a few key tokens, which may not be effectively captured using the standard generation objective where each token contributes equally to the overall loss. Therefore, to encourage the generator to produce label-discriminative samples, \cite{meng2023tuning} train the original model via weighted maximum likelihood where the weight of each token is automatically adjusted based on a discriminative meta-learning objective. Aimed at reducing the risk of memorization for fine-tuning with sensitive data, \cite{kurakin2023harnessing} involves the technique of Differential Privacy (DP) in the tuning process to prevent data leakage during the fine-tuning stage.

% Decoding Strategies.
% multiple-path decoding, greedy decoding, stochastic decoding, nucleus sampling

% \subsection{Procudure Design}
% In addition to the above two methods of directly interacting with LLMs to improve their response quality, many studies have realized that rather than treating LLM as a one-stop service that ``takes requirements as input and outputs the desired synthetic data'', we can also manually schedule and optimize its workflow through methods like data preparation at the early stage and task decomposition, etc. Such a systematic design can reduce the workload of a single LLM, but also facilitates the injection of human prior knowledge to assist in data generation.

% \subsubsection{Data Preparation}
% Valid supervision data are needed for either in-context learning or model fine-tuning. However, considering that raw data usually come with noise or in irregular forms, specific data preparation before actual employment is still necessary to ensure the model's understanding of data while maximizing the effectiveness of data utilization.

% \paragraph{Data Preprocessing.}
% For data not represented in natural language such as structured tabular data, we need to convert them into a form that LLMs can understand before we can provide them as inputs to the LLMs. Except for simply molding tabular data into a sentence structure closely resembling natural language, 
% \textcolor{blue}{\cite{zhao2023tabula} also explores techniques including token sequence compression and middle padding to optimize the training speed and ensure alignment of token sequence lengths across the entirety of the dataset, respectively.}

% \paragraph{Selective Annotation.}
% In LLM annotation tasks, we are usually provided with a large-scale unlabeled sample pool. However, with a limited budget or computational resources, we need to select the most informative inputs that are useful for downstream applications from the potentially noisy sets. \cite{ZhangLMZ023} covers some common selection strategies including random selection, maximum entropy selection, least confidence selection and $k$means selection for thorough comparisons. 
% \begin{equation}
%     11111
% \end{equation}
% Results show that uncertainty-based methods, i.e. maximal entropy and least confidence, perform significantly better than the random baseline, with faster convergence and better performance of the downstream model trained on the annotated data. Similarly, \cite{abs-2306-15766} also compares several different sampling rules and observes that annotations with LLM are best under base-inconsistent-sampling, where examples that hold the highest MSE error on base model predictions are selected to be annotated. Correspondingly, \cite{abs-2306-15766} develops an approximate metric for quantifying the degree of base-inconsistency of unlabeled inputs to avoid the need for knowledge of the ground truth labels of inputs.
% \cite{SuKWSWX0OZS023} instead proposes a novel unsupervised, graph-based selective annotation method named vote-$k$, to select diverse and representative examples to annotate.

% Besides, considering that LLMs' zero-shot performance still falls short on more difficult and pragmatic tasks compared to human performance \cite{wang-etal-2021-want-reduce,KoconCKKSBBGJKKKMMOPRWWK23}, \cite{LiSZKCLY23} utilizes uncertainty to estimate LLMs’ annotation capability to effectively allocate the annotation work among humans and LLMs, achieving both quality and cost objectives.

% \subsubsection{Task Decomposition}
% When facing complex tasks with specific requirements for generated data, due to insufficient logical analysis capabilities, the LLMs often cannot figure out a reasonable synthesis pipeline to obtain data that meets the requirements. At this point, if we can manually decompose the task into simpler sub-tasks that better leverage the advantages of LLMs, making the generation process more reasonably scheduled, it will greatly enhance the effectiveness of the generated data. 

% In common multi-text data generation tasks where several segments of text that are strongly related to each other are required, a popular solution is multi-step generation. Instead of letting LLMs generate a complete synthetic sample in one go, \cite{abs-2212-08635,DBLP:conf/emnlp/YeLK023,WangKMLSKH23} generates different parts of the sample in a step-by-step manner, and conditions each step on the previously generated content. Following a similar concept, S3 \cite{WangZS23} completes the generation of the entire dataset through multiple iterations, where each iteration is a targeted supplement to the data obtained in the previous step. \cite{HonovichSLS23} instead collects a large dataset of creative and diverse instructions named Unnatural Instructions, with consecutive generation from scratch and further expansion by rephrasing the generated ones. 

% For data that need to meet multiple demands simultaneously, one commonly used idea is to design different sub-tasks for different requirements. For instance, Explore-Instruct \cite{WanHYQB023} models the domain space as a tree structure and obtains comprehensive domain-specific instruction-tuning data following a search algorithm that comprises two fundamental operations: lookahead exploration and backtracking exploration, which promote the coverage of the generated data by pursuing fine-grained task decomposition and inclusiveness of different task categories within the domain, respectively. Similarly, Synthetic Prompting \cite{ShaoGSHDC23} alternates between a backward and forward process to generate high-quality data, which ensures that the question is both answerable and well-deﬁned and reﬁnes the reasoning chain to be more precise and consistent with the question, respectively. To obtain training materials that are both non-evasive and relatively harmless, Constitutional AI \cite{abs-2212-08073} first leverages an LLM to generate responses to ``red teaming'' prompts eliciting harmful samples, and then asks the model to critique its own response according to the given constitution, and then revise the original response in light of the critique.

% The idea of task composition can also be applied to solve difficult tasks where a single LLM is not sufficient to complete, by promoting collaboration between different models or algorithms. In highly subjective annotation tasks, instead of directly asking the LLMs to predict the labels of the given samples, \cite{abs-2205-02318} leverages heuristic prompts that are encapsulated as prompted labeling functions together with the label maps to extract various properties of the provided samples, which can be plugged into many standard weak supervision frameworks. In such frameworks, the labeling functions are executed on all the available unlabeled data to produce votes on what the correct label is. These votes are aggregated in the label model that produces probabilistic estimates of the correct label. For generating long dialogue instances, \cite{Mohapatra0CJ21} uses two LLMs to act as the user and the agent, respectively, the dialogues between which are then used to boost the publicly available datasets in low-resource settings. Moreover, to generate substantial samples to teach a model how to use external tools via simple APIs while requiring nothing more than a handful of demonstrations for each API, Toolformer \cite{abs-2302-04761} first samples a position $i$ and corresponding API call candidates $c_i^1,c_i^2,\cdots,c_i^k$, then executes these API calls and filters out all those do not reduce the loss over the next tokens.

% \subsubsection{Inference Strategies}
% There are some other tricks during the inference of the LLMs that can also optimize the utilization of the LLMs as a part of the entire data generation system. Except for selecting a proper decoding strategy to promote data diversity while ensuring their faithfulness, we also need to decide how much data we need to generate exactly for the best trade-off between inference cost and data availability. Considering that the synthetic data usually come with noise and require further filtering before being actually employed, the basic idea is that over-generation is generally performed to ensure that there is still enough usable data after removing dirty ones. Another reason for over-generation is that we need a larger quantity to compensate for the quality shortcomings of synthetic data compared to real data. Over-generation can serve not only to ensure there is enough data to support downstream tasks, but also as a foundation for subsequent techniques like consistency-based filtering, where the model's responses to the same input under different conditions can to some extent reflect the its confidence in the answer given.

% % pre-conditioning \cite{BorisovSLPK23}

% We created a new chat session for every tweet to ensure that the ChatGPT results are not influenced by the history of annotations \cite{abs-2303-15056}

==> wfgpdzfdwdyxvfnvwdgfyvxthbhxjbsd/sec/4_data_curation.tex <==
\subsection{Data Curation}
\label{sec:data_curation}
After the preceding steps, one may excessively generate overflowing and theoretically unlimited data $\mathcal{D}_\text{gen}$. However, these datasets often comprise a considerable portion of noisy, worthless, or even toxic samples, which primarily stems from two causes. Firstly, LLMs can inevitably produce corrupted samples with incorrect labels due to the hallucination problem. Secondly, ineffective prompts containing ambiguous descriptions can trick the model into generating irrelevant or redundant samples. Consequently, directly utilizing these low-quality data without proper processing may have a significant negative impact. 

To address this, plenty of data curation approaches have been studied, which mainly fall into two dominant groups of \textit{high-quality sample filtering} and \textit{label enhancement} as elaborated below. 

% Notably these techniques are mostly orthogonal and can be integrated for boosted performances.

% \begin{itemize}
%     \item {\textbf{Sample filtering} methods aim to select a valuable subset with higher quality from the unprocessed set based on different heuristic metrics or re-weighting functions.}
%      \item {\textbf{Label enhancement} approaches focus on the refinery of potentially incorrect annotations through human intervention or auxiliary knowledge distillation.}
%       \item {\textbf{Robust training} employs robust learning techniques to implicitly mitigate the adverse effects of low-quality samples during downstream deployment. }
% \end{itemize}
% Notably these different groups of techniques are mostly orthogonal and can be integrated for boosted performances.

\begin{figure}[!t]
\centering
\includegraphics[width=1\linewidth]{fig/curation.pdf}
\caption{Two dominant approaches of data curation.}
\label{fig:curation}
\end{figure}

\subsubsection{High-Quality Sample Filtering} 
Sample filtering aims to weed out undesired low-quality samples and obtain a more helpful subset $\mathcal{D}_\text{curated}\! \subset\!\mathcal{D}_\text{gen}$. These methods typically design \textit{heuristic criteria} or \textit{re-weighting functions} to rerank samples for filtering, as shown in Figure~\ref{fig:curation}.

\paragraph{Heuristic Metrics.}
For methods based on heuristic metrics, the key step is to design appropriate criteria based on the learning dynamics, such as confidence score \citep{seedat2023curated}, influence function \cite{ye-etal-2022-progen}, and generation ability \cite{DBLP:conf/nips/MengHZH22}. SuperGen \cite{DBLP:conf/nips/MengHZH22} employs the estimated generation probability to identify samples most related to the desired label. \citet{seedat2023curated} discard samples with both low confidence and low uncertainty. Some other methods assume that clean samples are prone to hold similar predictions under different conditions and employ cross-condition consistency for filtering. Specifically, such consistency can be between LLM and downstream classifier \cite{yu-etal-2023-regen}, between multiple executions \cite{ye-etal-2023-generating}, or between neighboring data points \cite{seedat2023curated}. \citet{abs-2307-08701} leverage the powerful text understanding capabilities of LLMs to assess the quality of different samples and filter out those with low scores. Results show that Alpagasus~\cite{abs-2307-08701}, trained on a much smaller but curated dataset, surpasses the original Alpaca~\cite{alpaca} across several benchmarks, underscoring the importance of data curation.

% ReGen \cite{DBLP:conf/acl/YuZZ0SZ23} utilizes the consistency between LLMs and a downstream classifier, only preserving the samples with consistent predictions. SymGen \cite{DBLP:conf/emnlp/YeLK023} incorporates an agreement-based verifier that hinges on the agreement among multiple executions or formatting. In \cite{seedat2023curated}, the consistency between neighboring data points is leveraged to discard those samples whose labels conflict with their neighbors.

\paragraph{Sample Re-Weighting.}  
On the other hand, re-weighting methods believe all data are valuable but with varying importance.
Thus, they assign larger weights to correctly annotated or influential samples during downstream utilization \cite{zhang-etal-2023-llmaaa,GaoPLXY0ZLLK23,meng2023tuning}. For instance, SunGen \cite{GaoPLXY0ZLLK23} proposes an adaptive bi-level re-weighting algorithm without human annotations. FewGen \cite{meng2023tuning} designs a discriminative meta-learning objective to adjust sample weights and demarcate the nuanced differences between different labels.

% \paragraph{Consistency based.} 

\subsubsection{Label Enhancement}
{Label enhancement} methods strive to rectify the potentially erroneous annotations in generated samples. Due to confirmation bias, it is unrealistic for LLMs to identify their own mistakes. To address this, recent works either rely on \textit{human intervention} or incorporate a student model for \textit{human-free knowledge distillation}. 

\paragraph{Human Intervention.}  
A straightforward strategy for label refinery is to include human efforts to re-annotate the corrupted samples \cite{chung-etal-2023-increasing,wang-etal-2021-want-reduce,DBLP:journals/corr/abs-2306-00176}. \citet{wang-etal-2021-want-reduce} proposed to actively select samples with the lowest confidence for human re-labeling. \citet{DBLP:journals/corr/abs-2306-00176} and \citet{liu-etal-2022-wanli} further emphasize the importance of human review and suggest comparing annotations from humans and LLMs guided by the same codebook. Despite the simplicity, these methods can lead to considerable labeling costs and can be unrealistic in practical deployment. 

% \cite{DBLP:conf/acl/ChungKA23} introduces two human intervention strategies of label replacement and out-of-scope filtering to correct misaligned labels and remove unrelated samples respectively. 
\paragraph{Auxiliary Model.}
To reduce the labeling cost, a more pragmatic human-free paradigm is developed which involves auxiliary student models for knowledge distillation and label refinery \cite{xiao-etal-2023-freeal,DBLP:journals/corr/abs-2311-08640,saad-falcon-etal-2023-udapdr}. These methods rely on the weakly supervised ability of student models and hypothesize that a student distilled from the LLM teacher can produce superior labels. The seminal work FreeAL \cite{xiao-etal-2023-freeal} proposes a collaborative framework, where a student model is leveraged to distill the high-quality task-related knowledge from the weak annotations and in return feedback LLMs for label refinery. MCKD \cite{DBLP:journals/corr/abs-2311-08640} designs a multistage distillation pipeline with data-split training and cross-partition labeling to avoid overfitting on noisy labels. With the expanding abilities and availability of LLMs, the incorporation of auxiliary student models will play a more crucial role as a cost-effective alternative to human intervention.

% collaborative training and distillation of small models will become more crucial in acting as a low-cost substitute for human annotation.

% Through these collaborative iterations between the LLM and student model, the high-quality task-specific knowledge is distilled to revise the annotations.


% \subsubsection{Robust Training Techniques}
% Robust training serves as an implicit curation paradigm to reduce the negative impact of low-quality data during downstream deployment. Among these robust learning techniques, label smoothing \cite{DBLP:conf/nips/MengHZH22}, temporal ensembling \cite{DBLP:conf/icml/MengMHZA023}, noise-tolerant losses \cite{DBLP:conf/iclr/GaoPLXY0ZLLK23,DBLP:conf/emnlp/YeG0F0K22}, and prediction ensemble \cite{DBLP:journals/corr/abs-2303-16854} are the prominent ones. Please refer to \cite{zhou2018brief} for more details. It is worth noting that these methods do not explicitly revise the generated data, but rather employ robust techniques to alleviate the impact of low-quality data.

% Label smoothing \cite{DBLP:conf/nips/MullerKH19} is a regularization to prevent overfitting on noise where the label is replaced with a mixture of one-hot vector and uniform distribution. Temporal ensembling \cite{DBLP:conf/iclr/LaineA17} maintains a consensus prediction using outputs in different epochs to suppress fluctuation. Noise-tolerant losses \cite{DBLP:conf/iclr/ZhangBHRV17,DBLP:conf/emnlp/YeG0F0K22} are designed to achieve a small and unbiased risk for clean data and enhance noise tolerance. Prediction ensembling \cite{DBLP:journals/corr/abs-2303-16854} leverages multiple LLMs or prompts in parallel and integrates their predictions for improved robustness. It is worth noting that these methods do not explicitly revise the generated data, but rather employ robust techniques to alleviate the impact of low-quality data.
% % \subsubsection{Label smoothing}
% % \subsubsection{Temporal ensemble}
% % \subsubsection{Noise-tolerant losses}


==> wfgpdzfdwdyxvfnvwdgfyvxthbhxjbsd/sec/5_data_evaluation.tex <==
\begin{figure}[!ht]
\centering
\includegraphics[width=1\linewidth]{fig/evaluation.pdf}
\caption{Direct and indirect methods of data evaluation.}
\label{fig:evaluation}
\end{figure}

\subsection{Data Evaluation}
Before the employment of generated data, it is important to evaluate the quality and application effectiveness of the data, to ensure its value to downstream tasks. 
The current mainstream evaluation methods can be roughly divided into two categories: \textit{direct} and \textit{indirect}, which evaluate the quality of $\mathcal{D}_\text{gen}$ individually and through its effectiveness on downstream tasks, respectively.
% Consequently, there is an urgent need to employ reliable evaluation methods for a comprehensive assessment of the data. The most direct assessment is to evaluate the data itself $\mathcal{D}_\text{gen}$, which visually presents various information but can be challenging when it comes to quantifying data effectiveness. Therefore, in addition to direct evaluation, indirect evaluation is employed by training models with the data and subsequently evaluating those models $\mathcal{M}^{gen}_\theta$.
% After obtaining processed data, a reliable evaluation mechanism is necessary to assess the data. 

% \subsubsection{Generated Data Evaluation}
\subsubsection{Direct Evaluation}

\paragraph{Data Faithfulness.}
Ideally, automatic evaluation of the LLMs' generation results can be easily realized with ground truths from existing datasets, if available \cite{abs-2304-10145}. However, for open-ended data, human-based evaluation is necessitated. A straightforward idea is to provide some generated samples to human experts, who will then determine whether they are correct, according to which we can estimate the overall generation quality \cite{WangKMLSKH23}. Theoretically, the larger the sample size, the more accurate the estimation results will be, but the labor it costs will correspondingly get higher. To this end, a reliable auxiliary model can be leveraged for a more comprehensive yet cost-effective evaluation of the generated data in replace of human experts~\cite{DBLP:conf/acl/ChungKA23}. Considering that most models can only process contents of limited length, appropriate information extraction can reduce the burden of the auxiliary model and contribute to a more precise prediction of whether a sample contains factual errors \cite{lee2022factuality}.

\paragraph{Data Diversity.}The quantification of data diversity primarily employs vocabulary statistics and sample relevance calculations. Vocabulary statistics~\cite{abs-2306-15895}, such as vocabulary size and N-gram frequency, provide a straightforward and intuitive approach. However, they struggle to capture the semantic information of a dataset. The calculation of sample relevance compensates for this limitation effectively. The most common measures of sample correlation are based on cosine similarity~\cite{WangZS23} and sample distance~\cite{DBLP:conf/acl/ChungKA23}, which can better capture the contextual and semantic diversity of the dataset. Furthermore, these metrics can also be leveraged to select in-context demonstrations $e_\text{demo}$~\cite{WangKMLSKH23} that are more dissimilar with the previously generated samples, thereby leading to more diversified generation results.

% \subsubsection{Generated Data Performance Evaluation}
\subsubsection{Indirect Evaluation}
\paragraph{Benchmark Evaluation.}
The performance of downstream models trained on the generated data can also reflect the generation quality to some extent~\cite{abs-2306-15895,DBLP:conf/acl/ChungKA23}. 
% Through comparing models trained on different datasets, \citet{abs-2306-15895} demonstrates that LLMs can generate new data that complements the original data effectively in text classification tasks. 
Specifically, the impact of synthetic data can be evaluated from multiple dimensions except for the specialized capabilities of the downstream models. For example, TruthfulQA enables the assessment of a model's ability to identify true claims \cite{abs-2305-03047}; NIV2 is employed to evaluate a model's language comprehension and reasoning abilities across multiple tasks \cite{WangKMLSKH23}. 

\paragraph{Open Evaluation.}
For open-ended benchmarks, evaluation by humans or auxiliary models is necessitated due to the absence of standardized answers. To fully leverage the preference outputs of the auxiliary models, multiple evaluation strategies have been designed, such as response ranking~\cite{abs-2304-12244}, four-level rating system~\cite{WangKMLSKH23} and Elo scores~\cite{abs-2212-08073}. To further reduce evaluation costs, \citet{abs-2305-03047,abs-2304-12244} utilize the automatic evaluation framework based on GPT-4 proposed by Vicuna for evaluation. However, general LLMs may lack enough knowledge for domain-specific tasks, which hinders them to provide effective evaluation~\cite{bran2023chemcrow}. Therefore, collecting human assessment data to fine-tune open-source models for evaluation purposes is an important practice in real-world scenarios~\cite{abs-2303-16854}. Other techniques like~\cite{peng2024energy,peng2023came} remain to be further explored.

% \subsection{Generated Data Evaluation}
% For generated data, the most direct evaluation involves assessing the quality of the data itself. This can be accomplished by annotating the data on existing datasets to verify the accuracy of the annotation results~\cite{abs-2303-16854,zhu2023can}. However, for open-ended data, human-based evaluation is commonly employed~\cite{WangKMLSKH23}. Due to the high cost associated with human-based evaluation, \cite{DBLP:conf/acl/ChungKA23} evaluates synthetic data using a model trained on original data. Additionally, the Remote-Clique metric is employed to quantify the diversity of data~\cite{DBLP:conf/acl/ChungKA23}. The chamfer distance score~\cite{LiZL023}, vocabulary size~\cite{abs-2306-15895}, and n-gram statistics~\cite{abs-2306-15895,lee2022factuality} are also employed for analyzing the diversity of data. It is observed that as the subjectivity of the task increases, the dissimilarity in data diversity between real-world and generated data becomes more pronounced~\cite{LiZL023}. LLMs can be utilized to assess the difficulty and complexity of instructions~\cite{abs-2304-12244}, but it requires the formulation of sound strategies to alleviate model misjudgments. To investigate the disparities between generated and original data, MAUVE~\cite{kurakin2023harnessing}, cosine similarity~\cite{wang2023let}, and ROUGE-L~\cite{WangKMLSKH23} are employed. To analyze the factuality of data, \cite{lee2022factuality} compares it with real-world facts from the perspectives of entity and textual entailment, demonstrating a positive correlation between model size and the factuality of data.

% \subsection{Generated Data Performance Evaluation}
% Generated data is frequently employed in model training, allowing for the quantification of data impact through the evaluation of the model. \cite{kurakin2023harnessing,abs-2306-15895,wang2023let,LiZL023,DBLP:conf/acl/ChungKA23} apply models trained on generated data to downstream tasks, comparing the performance of models trained on various datasets. Through comparing models trained on different datasets, \cite{abs-2306-15895} demonstrates that LLMs can generate new data that complements the original data effectively in text classification tasks. In addition to assessing the model's performance in downstream tasks, BBH (a subset of BIG-bench) is employed for evaluating the model's general capabilities~\cite{WangKMLSKH23}. TruthfulQA enables the assessment of a model's proficiency in identifying true claims~\cite{abs-2305-03047}. HH-RLHF can be utilized to evaluate the model's harmlessness and helpfulness~\cite{abs-2309-00267}. For open-ended benchmarks, evaluation is necessitated by human or models due to the absence of standardized answers. Response ranking~\cite{abs-2304-12244}, four-level rating system~\cite{WangKMLSKH23}, and Elo scores~\cite{abs-2212-08073} are employed to evaluate model outputs using artificial preference. \cite{abs-2305-03047,abs-2304-12244} utilize the automatic evaluation framework based on GPT-4 proposed by Vicuna for evaluation. To mitigate order bias, \cite{abs-2304-12244} alternate the placement of different model response outcomes in pairwise comparisons. However, relying on the evaluation with closed-source LLMs depends on the model's internal knowledge, making it challenging to ensure the effectiveness of the evaluation when the model has limited understanding of domain knowledge~\cite{bran2023chemcrow}. Therefore, it is possible to collect human assessment data and fine-tuning open-source models for evaluation purposes~\cite{abs-2303-16854}.

==> wfgpdzfdwdyxvfnvwdgfyvxthbhxjbsd/sec/7_discussion_conclusion.tex <==
% 1. 大模型的知识有long-tailed。如果没有人类干预，那么大模型会生成的biased的结果，这也是为什么data syn需要远超真实数据的样本才能达到接近的performance。
% 2. human定义的prompts、instructions可以一定程度上缓解，但是实际上最直接的可能还是依赖人力去提供真实的样本、标注或其他知识。
% 3. 要讨论哪些呢？
% a. 人类要在大模型生成的哪些生命周期介入？
% b. 一个人机友好的数据生成系统应该怎样设计？
% c. 人类的介入成本要如何控制？
% 总体地讲解一下在真正应用的时候值得注意的方向，
% Below, we will discuss from the perspectives of human-machine collaboration and complex task decomposition.
% While current solutions show good performance, manual synthesis remains the primary method for generating complex data. In addition, incorporating relevant knowledge aids accurate feedback \cite{abs-2311-00287}, but effectively filtering information for LLM is still an area requiring exploration. Simultaneously, human guidance improves data generation quality, but constructing human-machine collaborative modes needs further discussion. 
% Below, we will discuss the three perspectives mentioned above.
\section{Future Directions}

\subsection{Complex Task Decomposition}
% Current research in multi-step generation algorithms primarily focues on relatively straightforward tasks such as named entity recognition, and rely heavily on manually designed decomposition procedures. 
% However, many real-world scenarios involve considerably more intricate data generation processes.
Current multi-step generation algorithms depend on the model's understanding of task requirements, requiring it to perform complex logical reasoning with limited information. However, in real-world complex scenarios, this limited information may not adequately support effective decision-making.
For instance, the generation of mathematical problem-solution pairs entails multiple reasoning steps and may necessitate the utilization of calculator tools for validation. 
To date, there remains a lack of systematic investigation on how to activate the reasoning and planning capabilities of LLMs for autonomous synthetic data generation. 
Inspired by prevalent LLMs-based agents like HuggingGPT \cite{DBLP:journals/corr/abs-2303-17580} and MetaGPT \cite{DBLP:journals/corr/abs-2308-00352}, we believe it would also be quite valuable to develop a data generation \textit{agent} for industrial applications.


\subsection{Knowledge Enhancement}
Recent research has found that LLMs' knowledge is long-tailed and biased \cite{DBLP:journals/jdiq/NavigliCR23,DBLP:conf/acl/FeiHCB23}. 
Lacking specific domain knowledge, LLMs tend to generate biased, monotonous, and even unfaithful data. 
Though we have introduced how to mildly guide the data generation with task specification and conditional prompting in the previous sections, such methods still hold strong limitations and are not conducive to scalable implementation. 
Instead, we believe that developing automated condition controls directly on mature domain knowledge bases will significantly improve the efficiency of knowledge enhancement. 
For example, we can establish certain links between the LLMs and external knowledge graphs \cite{DBLP:journals/tnn/JiPCMY22} or retrieve augmentation from the website \cite{DBLP:journals/corr/abs-2312-10997}, which is helpful for the definition, decomposition, and reasoning of data features throughout the entire generation process. Additionally, with enhanced domain knowledge, we may also better assess the quality of generated data or even develop automatic evaluation systems. Overall, we believe that knowledge-driven data generation will be a key focus for future studies.

\subsection{Synergy between Large \& Small LMs}
% 在上文中，我们介绍了可以利用特定领域的小模型来评估大模型的数据生成质量，从中我们可以窥见一个重要的研究方向是将这种自动化的性能评估实时反馈到数据生成的过程中，从而引导模型进行相应的修正和调整。FreeAL证明了，可以基于噪声标签学习中的小样本损失筛选技术，来自动化筛选标注数据。这说明，我们可以通过一体化的大小模型协同验证来低成本地Curate数据。然而，他们的工作仅仅探索了模型所提供的confidence的作用，未来我们希望能够看到基于小模型的更多不同输出信息与大模型进行协同来提升生成数据的质量。
In Section~\ref{sec:data_curation}, we introduced the use of small domain-specific models for data curation. In particular, FreeAL \cite{xiao-etal-2023-freeal} has shown the feasibility of low-cost data curation with integrated collaboration between large and small models. 
The idea of leveraging real-time feedback provided by automated performance evaluation during the data generation process to guide the corresponding adjustments in the following generation hints at an important research direction. 
However, the exploitation of small LMs at the current stage is simply based on prediction confidence. In the future, we are looking forward to seeing more diversified collaboration modes between large and small models to improve the quality of generated data, e.g.,  usage of various output information, new design of collaborative architectures, and so on. 

\subsection{Human-Model Collaboration}
Data, as the source of model intelligence, theoretically cannot be generated completely without human intervention. Otherwise, wild synthetic data that carries noisy, toxic information can easily ``poison'' a model, even resulting in mode collapse. Due to the inherent bias of LLMs, they can hardly be self-aware of the bias in their generated data and finally deviate from our intentions. Thus, designing a human-friendly interactive system to involves a few necessary human knowledge for annotation and verification is vital and irreplaceable. To date, there is still a lack of a generic framework to standardize and systematize the human-machine collaboration involved in the data production process. 

We believe that an appropriate design of such a system must be based on a thorough understanding of the strengths and limitations of human intervention, and should follow the human-centered principle. To achieve sustainable and efficient human involvement, we need comprehensive consideration of various factors such as feasibility, cost, and even labor psychology. For specific examples: (i)-readability and interpretability of the information provided by the LLMs should be ensured to reduce obstacles to human understanding; (ii)-upstream knowledge enrichment or filtering should be carried out to improve the efficiency of human resource utilization and reduce consumption on tasks with low cost-effectiveness; (iii)-incorporating enjoyable interactive features can not only mitigate the negative impact of mechanical data processing tasks on humans but also attract a broader audience.

% \subsection{Complex Task Decomposition}
% % Current research in multi-step generation algorithms primarily focues on relatively straightforward tasks such as named entity recognition, and rely heavily on manually designed decomposition procedures. 
% % However, many real-world scenarios involve considerably more intricate data generation processes.
% \textcolor{red}{Current multi-step generation algorithms depend on the model's understanding of task requirements, requiring it to perform complex logical reasoning with limited information. However, in real-world complex scenarios, this limited information may not adequately support effective decision-making.}
% For instance, the generation of mathematical problem-solution pairs entails multiple reasoning steps and may necessitate the utilization of calculator tools for validation. 
% To date, there remains a lack of systematic investigation on how to activate the reasoning and planning capabilities of LLMs for autonomous synthetic data generation. 
% \textcolor{red}{Inspired by prevalent LLMs-based agents \cite{} like HuggingGPT and MetaGPT, we believe it would also be quite valuable to develop a data generation agent for industrial applications. }

% % The majority of datasets related to complex tasks rely heavily on human annotation~\cite{abs-2305-08322}. 
% % LLMs exhibit limited effectiveness in directly generating answers~\cite{lee2022factuality}. However, task decomposition~\cite{abs-2307-16789} based on ICL demonstrates promising potential, while also creating conditions for fine-grained evaluation. Nevertheless, in each decomposed step, the length of incoming information increases with the addition of the preceding steps \cite{abs-2307-16789}. The design of a loosely coupled, structured framework becomes a topic for discussion, aiming to mitigate the strong correlation between the length of received information and the number of steps. Meanwhile, the task decomposition granularity, step regression, and task termination rely on the LLM's understanding of tasks. Humans guide the LLM solely through the establishment of principles and the construction of examples. Exploring the creation of more interesting interaction principles and selecting more effective examples remains worthy of investigation.


% \subsection{Knowledge-Enhanced Data Generation}
% % The prerequisite for generating accurate data is the presence of sufficient prior knowledge. Confronted with unknown information in an open-world scenario, injecting effective knowledge aids the model in providing accurate feedback for complex tasks~\cite{abs-2311-00287}. However, the exploration of how to selectively filter information~\cite{FuZWQZ23} that is effective for LLM remains a subject for investigation. 
% % Numerous efforts are focused on filtering knowledge highly relevant to specific goals, with relatively less discussion regarding semantic conflicts in knowledge. When presented with multiple pieces of information that are inconsistent, LLM tends to favor information consistent with its own memory, which contradicts the original intent of knowledge injection \cite{Xie2024KnowledgeConflict}. Particularly when dealing with time-sensitive knowledge, such as descriptions of the same event under different temporal conditions, this tendency can lead to catastrophic consequences. Additionally, the detection of conflicts in knowledge themes can assist in the fine-grained screening of irrelevant knowledge. Therefore, before injecting knowledge, it is crucial to establish an auditing mechanism to prevent situations of knowledge conflict.
% There has been some work indicating that the knowledge of LLMs is long-tailed. 
% When presented with multiple pieces of information that are inconsistent, LLM tends to favor information consistent with its own dark knowledge.

% % There has been some work indicating that the knowledge of LLMs is long-tailed. 
% % When presented with multiple pieces of information that are inconsistent, LLM tends to favor information consistent with its own dark knowledge, which contradicts the original intent of knowledge injection \cite{Xie2024KnowledgeConflict}. 
% % Therefore, the LLMs typically generate biased data when lacking proper control. 
% % This can be alleviated by knowledge injection techniques such as knowledge retrieved from 

% \subsection{Human-Machine Collaboration.}
% The knowledge distribution of LLM exhibits a long-tail characteristic, making it challenging to ensure strict professionalism of generated data, especially without human guidance. To achieve results closely resembling real data, a significantly larger volume of synthetic data is required than that of real data \cite{abs-2309-11674}. While the rules established by experts and the feedback from tools can enhance data quality, aligning human preferences and global rules through artificially generated professional data remains the most direct approach.

% It's known that human intervention is costly. To maximize data quality with a limited budget, we need to consider where to incorporate human-machine interaction in the data lifecycle. The most common practice is to involve human intervention during the data generation phase \cite{LiSZKCLY23}, but currently, there is a lack of a universal human-machine collaborative framework, and new methods to inspire a heuristic-driven generation of new data from manually annotated samples still need exploration. Relying solely on a few samples with human preferences can lead to monotony in generated trends. Therefore, during data evaluation, manual feedback is necessary to adjust the guiding principles of the LLM.

% In human-machine interaction design, it is essential to approach the design from a human-centric perspective to ensure the readability and interpretability of the information provided by LLM, thereby reducing the barriers to human comprehension. Additionally, incorporate entertaining interactive features for a more engaging data processing experience. This not only mitigates the negative impact of mechanical data processing tasks on humans but also attracts a wider audience, contributing to the creation of a sustainable and efficient data loop ecosystem.

% % While the current approaches based on model interactions~\cite{abs-2306-05301} and model self-iteration~\cite{abs-2304-12244} demonstrate significant potential in data generation, there still exists a noticeable gap when compared to human annotation~\cite{abs-2306-15895}. Moreover, in scenarios with minimal human intervention, the quality of generated data overly relies on the inherent capabilities of the model, making it challenging for less powerful models to produce high-quality data with only limited human guidance. To balance the generative effectiveness of the model and human engagement, \citet{LiSZKCLY23} discusses a framework for data annotation allocation, coordinating manual annotation with model-based annotation, but exhibits relatively weak adaptability to open-ended tasks with high subjectivity. Exploring a universal human-machine coordination framework to balance data quality and annotation costs will be an interesting investigation.

% % Meanwhile, \citet{bran2023chemcrow} observes that LLMs experience significant evaluation errors in the absence of relevant domain expertise. Sensitivity to input information and the "sycophancy" towards input information can all contribute to the instability of assessments based on LLM. Manual evaluation exhibits drawbacks in terms of both assessment efficiency and cost. Hence, there is a requirement for a more specialized and efficient evaluation method. If one can integrate the strengths of manual evaluation and model evaluation to develop a human-machine evaluation allocation mechanism or fuse domain knowledge and human assessment preferences into the evaluation model, it would be interesting to explore.

\section{Conclusion}
In this paper, we present a systematic review of advancements in synthetic data generation propelled by Large Language Models (LLMs). We aim to offer guidance to enterprises and organizations on effectively building their domain-specific datasets using LLMs. In the meantime, we endeavor to provide insights into the challenges and opportunities within this field, while also proposing potential directions for future research.
We hope that our work can promote the rapid production of large amounts of data in various fields and push the limits of data-centric AI. 
We also envision a fantastic future, where an LLMs community, endowed with human-like abilities such as bionics and communication, may be constructed to generate data for its own self-improvement.

% % In this work, we provide a comprehensive review of recent progress in generating high-quality data on LLMs. We summarize and analyze the data synthesis pipeline in terms of data generation, data curation, and data evaluation. While existing methods have demonstrated favorable performance, LLM-based data generation has experienced a relatively short development time and presents significant growth potential. 

% % For example-based guidance, data annotation, and data evaluation, large models can replace manual efforts in generating guiding examples, annotating samples, and quantifying performance. In the generation of high-quality data with emphasis on diversity and security, intricate principles and purposive rules still necessitate expert pre-specification~\cite{abs-2304-12244,abs-2307-16789,LiZ000YLHL23} to prevent data degradation. Moreover, within datasets currently synthesized by LLMs, the majority of seed data is meticulously crafted by human hands~\cite{abs-2305-03047,abs-2304-12244,WangKMLSKH23}. Therefore, reliance on human-guided generation is challenging to avoid in the generation process, yet real-time guidance involving human participation entails prohibitively high costs. Meanwhile, LLM has shown promising results in correcting generation preferences based on feedback~\cite{wang2023let}. Consequently, introducing multi-channel factual feedback on the foundation of low-cost human guidance is a promising guiding strategy, enabling real-time correction of model-generated content while incorporating human preferences. 

==> wfgpdzfdwdyxvfnvwdgfyvxthbhxjbsd/sec/limitations.tex <==
\section*{Limitations}
In this paper, we survey existing studies on LLMs-driven synthetic data generation, curation, and evaluation, proposing a generic workflow for real-world practice. Synthetic data generation is a broad topic that involves data and models of various modals, including vision and speech. Due to the page limit, we mainly focus on the objective of text data and LLMs-driven approaches, while leaving investigations in other fields for future work. We will also keep paying attention to the latest work and add more related approaches with more detailed analysis.

\section*{Ethics Statement}
We believe that our proposed workflow of LLMs-driven synthetic data generation, curation, and evaluation can benefit both researchers who are interested in data-centric AI and industrial producers who are facing data problems. However, the malicious use of such synthetic data also raises ethical concerns that should arouse our vigilance.

\section*{Acknowledgements}
This work is supported by the Pioneer R\&D Program of Zhejiang (No. 2024C01035), NSFC under Grants (No. 62206247), and the Fundamental Research Funds for the Central Universities  (No. 226-2024-00049).



==> wfgpdzfdwdyxvfnvwdgfyvxthbhxjbsd/sec/preliminary.tex <==
\section{Preliminaries}
\subsection{Problem Definition}
The automated data generation pipeline is driven by a pre-trained LLM $\mathcal{M}_{\theta}$ with parameter $\theta$. We are initially given a particular target task $\mathcal{T}$ with label space $\mathcal{Y}$ and an optional small reference set $\mathcal{D}_\mathit{ref}=\{(x_i,y_i)\}_{i=1}^{N}$ that can be either labeled or unlabeled.  The primary goal is to harness the capabilities of $\mathcal{M}$ to induce samples $(x^\mathit{gen},y^\mathit{gen})$ where $y^\mathit{gen}\in\mathcal{Y}$ and then constitute a synthetic dataset $\mathcal{D}_\mathit{gen}=\{(x_i^\mathit{gen},y_i^\mathit{gen})\}_{i=1}^{N_\mathit{gen}}$ :
\begin{equation}
    \mathcal{D}_\mathit{gen} \leftarrow G(\mathcal{M}_\theta, \mathcal{T}, \mathcal{D}_\mathit{ref})
    \label{eq:overall}
\end{equation}
where $G$ is the overall generation algorithm. Under this unified framework, the generation pipelines can be divided into two types: \textbf{data synthesis} and \textbf{data annotation}, which is illustrated in Figure~\ref{}.
\begin{itemize}
    \item \textbf{Data Synthesis} employs LLMs as generators to create new fictitious samples.  Given label-specific prompt, $\mathcal{M}$ is steered to generate multiple data $\{x_i^\mathit{gen}\}_{i=1}^{N_\mathit{gen}}$ for  targeted class $y^\mathit{gen}$. 
    \item \textbf{Data Annotation} employs LLMs as labelers to annotate the existing unlabeled data. Given an unlabeled set $\mathcal{D}_u$, $\mathcal{M}$ is prompted to predict the label $y^\mathit{gen}$ for each unlabeled sample $x_u\in \mathcal{D}_u$ and the input-label pair constitute $\mathcal{D}_\mathit{gen}$.
\end{itemize}
Notably, both of these two paradigms can be integrated with demonstrations from $\mathcal{D}_\mathit{ref}$ for boosted performance, which can be samples of target class for data synthesis and relevant input-label pairs for data annotation. This is known as \textbf{few-shot} setting, whereas \textbf{zero-shot} setting denotes the situation without demonstration samples from $\mathcal{D}_\mathit{ref}$. 


\paragraph{Requirements of $\mathcal{D}_\text{gen}$.} Distinguished from data generation in a broad sense, in this paper we only investigate methods that can provide supervision information valuable to other downstream tasks through data flow, which raises specific requirements to the generated $\mathcal{D}_\text{gen}$ from the following three aspects:

\begin{itemize}
    \item \textbf{Faithfulness.}
    To provide valid supervision, the generated data firstly should be not only correctly labeled, but also both logically and grammatically coherent.
    \item \textbf{Diversity.}
    Limited by the inherent bias of LLMs, the generated contents usually tend to be monotonous. However, the distribution of real data often exhibits a high degree of diversity, which should also be reflected in the generated data for better alignment.
    \item \textbf{Coverage.}
    Domain coverage is another essential element to ensure the robustness of deploying $\mathcal{D}_\text{gen}$ in the downstream tasks.
\end{itemize}
